Concretization of Abstract Traffic Scene Specifications Using Metaheuristic Search

Existing safety assurance approaches for autonomous vehicles (AVs) perform system-level safety evaluation by placing the AV-under-test in challenging traffic scenarios captured by abstract scenario specifications and investigated in realistic traffic simulators. As a first step towards scenario-based testing of AVs, the initial scene of a traffic scenario must be concretized. In this context, the scene concretization challenge takes as input a high-level specification of abstract traffic scenes and aims to map them to concrete scenes where exact numeric initial values are defined for each attribute of a vehicle (e.g. position or velocity). In this paper, we propose a traffic scene concretization approach that places vehicles on realistic road maps such that they satisfy an extensible set of abstract constraints defined by an expressive scene specification language which also supports static detection of inconsistencies. Then, abstract constraints are mapped to corresponding numeric constraints, which are solved by metaheuristic search with customizable objective functions and constraint aggregation strategies. We conduct a series of experiments over three realistic road maps to compare eight configurations of our approach with three variations of the state-of-the-art Scenic tool, and to evaluate its scalability.

==> chp/dynamics.tex <==
\section{Towards scenario-based testing of AVs}

Although concrete initial traffic scenes may be useful to test certain (e.g. vision-based) components of AVs, they are not sufficient to evaluate their system-level safety.
A common approach to do so is scenario-based testing, where aside from an initial scene, a test case  requires the integration of temporal developments related to actors in a scenario, as well as evaluation criteria.
We propose a lightweight scenario generation approach that builds on the proposed initial scene concretization approach by assigning target traffic maneuvers and abstract speeds to actors in a scenario. 

% Once the initial scene is derived, the actors are augmented with dynamic behavior according to temporal constraints included in the functional scenario.
% Our proposed approach supports traffic maneuvers and speeds as abstract constraints: handling of more complex temporal (and causal) constraints, e.g. constraints representable through various temporal logic languages, is left for future work.

\todo{(1.1) Usefullness and Critical ScenGen -> (2.2) Dynamics as TC}
\todo{Mention this in 2.6 response.}

\begin{figure}[htp]
    \begin{center}
    \captionsetup{justification=centering}
      \includegraphics[width=\linewidth]{fig/elab/2stepOverview.png}
      \caption{Scenario-based AV test execution framework overview}
      \label{fig:2step}
    \end{center}
\end{figure}

\todo{I might want to improve this figure}

\textit{Scenario-based test execution overview}:
An overview of our proposed AV test execution framework is provided in \autoref{fig:2step}.
The framework takes as input a \fss{} (composed of a functional initial scene specification \fssInit{} and additional abstract temporal constraints collected in \fssTemp{}) and \textit{Test Evaluation criteria} for the ego-vehicle (the system-under-test).
As a first step, the \fssInit{} is fed into \textit{our proposed} \moopt{}\textit{-based approach} to yield a concrete initial scene.
Secondly, the concrete initial scene and the \fssTemp{} are input into a \textit{Temporal Property Assignment} process which assigns temporal properties to actors according to the temporal constraints contained in \fssTemp{}.
The \textit{Temporal Property Assignment} (\tpa{}) step yields a concrete (dynamic) scenario which can be simulated.

The concertized scenario and the input \textit{Test Evaluation Criteria} are then input into a \textbf{Test Simulation} framework which outputs the \textit{Test Outcome}.
Test evaluation criteria may be represented as high-level success criteria, such as \textit{The ego vehicle must not collide with any component throughout test execution}, or more precise requirements, as measured by oracles \cite{Jahangirova2021Oracle}, which may be derived from existing AV safety standards.
Nevertheless, in this paper, we focus on the scenario concretization portion of our proposed test execution framework.
As such, test simulation is considered as a black box.
\todo{I forgot to mention multiplicity!!!!}

\textit{Temporal property assignment}:
In order to derive concrete scenarios, our proposed framework assigns quasi-dynamic properties to actors.
Specifically, the \tpa{} component takes as input constraints that assign abstract maneuvers and an abstract speed to a single actor, and provides as output a simulation-ready concrete scenario with exact trajectories for the non-ego vehicles.
The ego-vehicle is assigned abstract target behavior which it must execute while satisfying the input \textit{test evaluation criteria}.

Note that conceptually, temporal constraints over actors may involve multiple actors (e.g.\textit{Actors A and B are getting closer to each other}) and may span over multiple temporal phases of a scenario execution.
However, handling such complex temporal constraints requires support for various temporal logic languges, which is outside the scope of this paper.

\todo[inline]{ADD AN EXAMPLE HERE? This would mean that I won't do anything related to this in the evaluation}

\textit{Usefulness of our scenario concretization approach}:
Our proposed scenario concretization approach takes as input arbitrary abstract scenes and provides a corresponding concretization.
As such, this paper does not focus on the properties of the abstract scenarios to be concretized.
Instead, it focusses on the properties of the concretization, given an abstract scenario as input.

In fact, our scenario concretization approach is meant to be used in parallel with (and not to replace) existing adversarial test scenario generation approaches \cite{TODO}.
Such a concretization approach is particularly beneficial as it allows to shift the reasoning about danger to a more abstract, human-understandable functional level, which is often how it is described in existing safety standards and among experts \cite{TODO}.
On the contrary, existing critical scenario generation approaches often provide low-level definitions of high-level safety concepts that are specific to the underlying technologies being used.
\todo{This last line is a draft, need to work on this}


% \todo[inline]{Our approach is meant to be used in parallel with existing critical scenaario gen appproaches, not meant to replace.}
% \todo[inline]{allows us to reason about such concepts like danger at a more abstract, human-understandable, level. we can separate the reasoning of danger from the numeric handling of the problem which has been shown 2 be beneficial in such application domains}
% \todo[inline]{Usefulness,}



% Our approach is meant to be used in collaboration with existing “adversarial” testing approaches
% The main advantage of our approach is that it allows us to reason about such concepts like danger at a more abstract, human-understandable, level. As such we can separate the reasoning of danger from the numeric handling of the problem which has been shown 2 be beneficial in such application domains.


\todo{(2.3) Critical ScenGen}
\todo{(2.1), (2.4) Do I wanna talk about vision-based things here??? bring the Section 6.8 stuff here...}


==> chp/reserve.tex <==


%%%%%%%%%%%%%%%%
GRACEFUL DEGRADATION
%%%%%%%%%%%%%%%%

% \todo{paragraph title for Graceful Degradation}
\subsection{Graceful degradation}
For complex scenes, a solution to a \mom~problem $M_{min}$ may not be found due to, for instance, inconsistent specifications or insufficient resources.
To address this issue, our proposed formalization allows the underlying \moopt~approach to provide an approximate solution as output, where only a subset of the distance functions in $M_{min}$ are minimised.
In this case, numeric constraints are treated as soft constraints, and the underlying \moopt~algorithm minimizes the distance function values to the best of its abilities within the limits of the allotted resources.
% (i.e. a UNSURE (pareto-optimal|aproximately satisfactory) solution is returned).
% \todo{choose wording of this last section}
% will provide a solution where the minimize the distance to satisfaction of all constraints (measured by distance functions) is minimized within the limits of alloted resources. 

% In factm in this case, numeric constraints 
% Note that 
% if no opt sol is provided, 
% partial solution to numeric problem, where some constraints are satisfied, and the distance to satisfzction is minimized
% in this case,constraints treated as soft constraints
% In this case, $c_i$ is treated as a soft constraint, which means that is no optimal solution is found, a non-optimal solution that may satisfy $c_i$ is returned.

Such graceful degradation is rarely provided by existing scene concretization approaches that handle generic scene specifications as input (e.g. where scenes are not limited to an a priori selected maneuver).
% \todo{might be missing something here}
% In fact, such approaches do not employ underlying optimization-based algorithms, thus graceful degradation
% \todo{make sure this is true}
For instance, rejection sampling used in \scenic~cannot provide an approximate solution if no solution is found.

% However, unlike in \scenic, our approach provides graceful degradation for the scene concretization problem: even if some functional relations are not satisfied, our approach will provide an approximately satisfactory solution. 

% \todo{given a numeric problem N, what is a candidate solutoin? What is a solution?}
% In order to solve a numeric problem N given as input, we propose a mapping to , 
% Given a numeric problem $N = \langle \actorSetI{N}, \constrSetI{N}, \roadmapI{N}, \dimensionsI{N} \rangle$
% A \moopt~algorithm is defined over a finite set of objectives . 
% We adapt a \moopt~approach to address a numeric problem  that corresponds to a scene concretization problem. 

\begin{figure}[htp]
     \centering
\captionsetup{justification=centering}
        % \begin{subfigure}[b]{0.75\columnwidth}
        %     \centering
        %     \includegraphics[width=\columnwidth]{fig/elab/QAs/gen-init-crop.png}
        %     \caption[]{Concrete scene where \textcolor{blue1}{\qaCanSeePred{\actorBl}{\actorR}}\\does not hold}%
        %     % {\textit{P1.0}: Object Diagram}    
        %     \label{fig:elab-init-sc}
        % \end{subfigure}
        
        \begin{subfigure}[b]{0.49\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{fig/elab/QAs/gen-partial-complete.png}
            % \caption[]{Scene semantically equivalent to \autoref{fig:elab-init-sc}}    
            \caption[]{A solution, \textcolor{blue1}{\qaCanSeePred{\actorFunG}{\actorFunBl}} holds}%
            \label{fig:elab-partial-complete}
        \end{subfigure}
        % \vskip\baselineskip
        \begin{subfigure}[b]{0.49\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{fig/elab/QAs/gen-partial-partial.png}
            \caption[]{An approximate solution, \textcolor{blue1}{\qaCanSeePred{\actorFunG}{\actorFunBl}} does not hold}      
            \label{fig:elab-partial-partial}
        \end{subfigure}
        
        \caption{Possible outcomes of our proposed approach, given \autoref{fig:func-full} as input. The \textcolor{blue1}{field of view of \actorFunG} is depicted.} 
        \label{fig:elab-concretizations-partial}
\end{figure}
\begin{exline}
We define a \mom~problem $M_{min}$ that corresponds to a numeric problem $N$ derived from the \fss~of \autoref{fig:func-full}.
\autoref{fig:elab-concretizations-partial} shows two possible outcomes of a \moopt~approach applied to $M_{min}$.
\autoref{fig:elab-partial-complete} depicts a concrete scene that fully complies with \autoref{fig:func-full} (i.e. it is a solution to $M_{min}$): all the numeric constraints included in $N$, hence all the functional relations in the corresponding partial model, are satisfied.
\autoref{fig:elab-partial-partial} depicts an approximate solution, where all functional relations hold, with the exception of \textcolor{blue1}{\qaCanSeePred{\actorFunG}{\actorFunBl}}.
Note that such an approximate solution cannot be derived by \scenic.
\end{exline}













%%%%%%%%%%%%%%%%
PARTIAL MODEL FORMALIZATION
%%%%%%%%%%%%%%%%

% A partial model is defined over a collection of objects $o_i$ according to \textit{relation assertions} which assign a 4-valued truth-value, one of \true, \false, \unk~(unspecified, may be either \true~or \false) and \err~(inconsistent, is \true~and \false~at the same time), to an \textit{n-ary} relation over a tuple of objects.

\textit{Syntax:}
\todo{Do I need a statement that every unspecified relation is unknown by default?}
% A partial model is defined over a finite set of objects $\dslObjectSet$ according to \textit{relation assertions} which assign a 4-valued truth-value, one of \true, \false, \unk~(unspecified) and \err~(inconsistent), to an \textit{n-ary} relation over a tuple of objects.
The syntax of a functional scene specification $FSSpec$ is defined as set of \textit{relation literals} over (a finite set of) variables $V$ using the relation symbols $\Sigma$ above.
% A relation literal can be (optionally) prefixed by the $\texttt{?}$ and $\texttt{!}$ symbols.
For example, $\qaFrontPred{v_1}{v_2}$ denotes that actor represented by variable  $v_2$ 
must be ahead of actor $v_1$.
%For example, $\qaFarPred{v_1}{v_2}$, $\texttt{!}\qaFarPred{v_1}{v_2}$,  and $\texttt{?}\qaFarPred{v_1}{v_2}$ denote that actors represented by variables 
%$v_1$ and $v_2$ must be, must not be or may be far from each other, respectively.

%respectively denote that the truth value of the predicate is \true, \false, \unk.

\textit{Semantics:}
The semantics of a functional scene specification is defined as a 3-valued partial model $P$ \cite{Semerath2017GraphConstraintEvaluation,sagiv2002parametric,Gopan04summarized}. 
More precisely, a relation $\qaBinaryPred{R}{v_1}{v_2}$ can be evaluated on a partial model $P$ by (1) mapping (binding) $Z\colon V\rightarrow\dslObjectSetI{P}$ variables to objects $\dslObjectSetI{P}$ of $P$, and (2) assigning a truth value (one of \true, \false, \unk) to each relation literal
(where the \unk~value signifies that the respective relation is uncertain or unspecified). Such a 3-valued semantic evaluation is denoted as $\semantics{\qaBinaryPred{R}{v_1}{v_2}}{P}{Z}$. For example, in the functional scene depicted in \autoref{fig:sceneAbsLevels}, the blue car is ahead of the red car, formally, $\semantics{\qaFrontPred{A_B}{A_R}}{P}{A_R \mapsto r, A_B \mapsto b}$
%For example, $\qaFarPred{v_1}{v_2}$

 

%(ranging over objects $\dslObjectSet$) according to \textit{relation assertions} which assign a 3-valued truth-value to an \textit{n-ary} relation over a tuple of objects.
%, one of \true, \false, \unk~(i.e. when the truth value is uncertain or unspecified), 

%$\qaFarPred{o_1}{o_2} : \false .$, or simply $\texttt{!}\qaFarPred{o_1}{o_2}$, states that there does not exist a \qaFar~relation between $o_1$ and $o_2$.
%Uncertainty is represented by the $\texttt{?}$ prefix.
% Note that the \texttt{?} prefix represents a truth-value \unk, while \texttt{!} and a lack of a prefix respectively represent \false~and \true.
% The semantics of such relations are evaluated in \cite{Semerath2017GraphConstraintEvaluation,sagiv2002parametric,Gopan04summarized}.


%Semantically, such a relation $\qaBinaryPred{R}{v_1}{v_2}$ can be evaluated on a partial model $P$ (defined over an object set $\dslObjectSetI{P}$) along a variable binding $Z\colon \{v_1,\ldots,v_n\}\rightarrow\dslObjectSetI{P}$.
%Such a semantic evaluation, denoted as $\semantics{\qaBinaryPred{R}{v_1}{v_2}}{P}{Z}$, results in a 3-valued truth value.


%%%%%%%%%%%%%% GRAPH PREDICATES
% A partial model may also be subject to graph predicates, defined as a set of relations (or their negation) in disjunctive normal form.
% For instance, \qaBinaryPred{VisDist}{$o_1$}{$o_2$} \texttt{:=} \qaFarPred{$o_1$}{$o_2$}, \texttt{!}\qaCanSeePred{$o_1$}{$o_2$}; defines a graph predicate \qa{VisDist} that states that object $o1$ is far from $o2$, and it cannot see $o2$.
% An error predicate adds an \err~prefix to a graph predicate, signifies that the predicate should never hold in a consistent model (i.e. it is asserted to \false).


%Currently, they are only evaluated over terms that represent actors of a scene (defined by their type, e.g. \qaCar~or \qaPedestrian), but our proposed approach may be generalized to components of the scenery as well.

% \todo{YES, cite Scenic here. Do I need to cite Scenic here? cuz they also propose something like this}
% \todo{Move this to after interpretation, and write a formalization}
% \todo[color=red]{scene spec is a graph where node is actor, each edge is labeled in accordance with the vocabulary}

% \textit{Partial Models:} In this paper, a functional scene specification corresponds to a partial model \cite{uncertain:definitions,uncertain:PartialModelAlloy}, which can represent uncertain (possible) elements of a scene.
% We use 3-valued logic where the traditional truth values \emph{true} ($\true$) and \emph{false} ($\false$) are extended with a third truth value $\unk$ to denote \emph{unknown} structural parts of the model \cite{Semerath2017GraphConstraintEvaluation,sagiv2002parametric,Gopan04summarized}.
% For traffic scenes, uncertainties are only applicable to relations (i.e. elements of $\Sigma$), and not to actors.

% Formally, a functional scene specification is represented as a logic structure $P = \logicModelTwo{\dslObjectSetI{P}}{\interpretationFun{P}}$,
% where $\dslObjectSetI{P}$ is the finite set of objects (each object corresponds to an actor),
% and $\interpretationFun{P}$ gives a 3-valued logic interpretation for each symbol $\dslStyle{s}\in\Sigma$ as $\interpretationFun{P}(\dslStyle{s}):(\dslObjectSetI{P})^{\alpha(\dslStyle{s})}\rightarrow \{\false,\true,\unk\}$, where $\alpha(\dslStyle{s})$ denotes the arity of $\dslStyle{s}$.



% %%%%%%%%%% FORMALIZATIONN INSTANCE
% \textit{Syntax:}
% A functional scene specification is represented textually as in \autoref{fig:func-full}.
% Such a representation collects a set of constraints interpreted in a binary manner, defined over a set of actors.
% If a predicate, or its negation, is included in the textual description, the interpretation of the corresponding predicate in the corresponding partial model representation is $\true$, or $\false$.

% \todo{concretizatoin is too early here??}
% Furthermore, constraints that are excluded from the textual representation may or may not hold in the concretization (i.e. they are interpreted to $\unk$ in the partial model).
% For instance, if no \textbf{distance constraint} is defined between actors \actorA~and \actorB, then all possible distance constraints between those actors (i.e. \qaClosePred{\actorA}{\actorB}, \qaMedPred{\actorA}{\actorB}, \qaFarPred{\actorA}{\actorB}) are interpreted to $\unk$, which means that in the concretization, \actorA~and \actorB may be separated by any distance.

% \todo[color=red]{represent scene as partial graph, we may wish to state the axioms (implications)}
% \todo[color=red]{say that input scene defines true links. so if a constraint is in the input scene, its true. and it has consequences (axioms) defined formally}
% The input of our approach is a functional-level scene specification defined as a collection of abstract constraints consistent with the constraint language proposed in \autoref{sec:pre-lang} defined over a set of actors.
% Actors are defined independently from the constraints.

% \todo{Move this to after interpretation, and write a formalization}
% In terms of semantics, In the case where constraints of every type do not exist between every pair of actors, we apply an open-world assumption..
% For example, if no distance constraint is defined between a pair of actors, then those two actors may be separated by \textit{any} distance.



%%%%%%%%%%%%%
Semanic differences between scenes
%%%%%%%%%%%%%
%%%%%%% MOTIVATION
\subsection{Semantic differences between concretizations}

\tododvab{Please check}
Functional scene specifications in existing safety standards are often limited to a relevant subset of constraints between actors (i.e. truth values for irrelevant constraints are not made explicit).
% A functional scene specification often only make explicit the  explicitly include constraints  corresponds 
% However, functional scenes often do not explicitly include truth values for all possible semantic relations between actors.
As such, multiple semantically different concrete scenes may correspond to the same functional scene specification.
By explicitly representing uncertainty, partial models define  equivalence classes for traffic scenes and may be used to reason about diversity and about semantic completeness at an abstract level.
% can natively handle coverage and diversity analysis over concrete scenes at an abstract level.

% A partial model defines an equivalence class for traffic scenes
% allow such coverage analysis by defining equivalence classes for traffic scenes.

% However, in terms of traffic scene concretization, existing safety standards often place coverage and diversity requirements over test suites containing traffic scenes.
% Coverage is addressed at an abstract level (note that changes at the concrete level pertainn to robustness properties).
% Thus, it is crucial to have a way to represent the semantic differences at an abstract level between concretizations of a same functional scene specification.
% Partial models natively represent uncertainty and they solve the problem by defining an equivalence class of traffic scenes.
% As such, we can reason about semantic completeness at the equivalence class level.

A concrete scene $CS$ derived from a functional scene specification $FS$ is defined as a concretization of the corresponding partial model $PM$.
Based on the concrete attributes of actors in $CS$, abstract relations (or their negation) are determined between them by using qualitative abstractions over the concrete scene.
This results in a concrete model $CM$, where each $\unk$~relation of $PM$ is concretised to $\true$ or to $\false$.
Once a concrete model is derived, scene generation approaches may increase the diversity of synthesised traffic scene test suites by guiding exploration towards new, semantically different scenes.
However, this is outside the scope of the current paper.

% This is a logical extension, which explain why we are setting things up like this, but outside the scope of this paper.

% Considering that a single functional-level scene corresponds to multiple concrete scenes

% Explicitly 
% Modeling uncertainty allows 
% multiple scenes that satisfy a same scene specification, but are semantically different.
% This is good for model generation, also it alows for covrage analysis
% instead of not carinf about the other things

% we can explicitly guide towards "different" TCs of the same scene spec


\begin{figure}[htp]
     \centering
\captionsetup{justification=centering}
        % \begin{subfigure}[b]{0.75\columnwidth}
        %     \centering
        %     \includegraphics[width=\columnwidth]{fig/elab/QAs/gen-init-crop.png}
        %     \caption[]{Concrete scene where \textcolor{blue1}{\qaCanSeePred{\actorBl}{\actorR}}\\does not hold}%
        %     % {\textit{P1.0}: Object Diagram}    
        %     \label{fig:elab-init-sc}
        % \end{subfigure}
        
        \begin{subfigure}[b]{0.49\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{fig/elab/QAs/gen-same-crop.png}
            % \caption[]{Scene semantically equivalent to \autoref{fig:elab-init-sc}}    
            \caption[]{Concrete scene where \textcolor{blue1}{\qaCanSeePred{\actorBl}{\actorR}} does not hold}%
            \label{fig:elab-same-sc}
        \end{subfigure}
        % \vskip\baselineskip
        \begin{subfigure}[b]{0.49\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{fig/elab/QAs/gen-crooked-crop.png}
            \caption[]{Concrete scene where \textcolor{blue1}{\qaCanSeePred{\actorBl}{\actorR}} holds}      
            \label{fig:elab-crooked}
        \end{subfigure}
        
        \caption{Concretizations of \autoref{fig:func-full}.\\The \textcolor{blue1}{field of view of \actorBl} is depicted.} 
        \label{fig:elab-concretizations-sc}
\end{figure}
\begin{exline}
\autoref{fig:elab-concretizations-sc} shows two concretizations of the functional scene specification provided in \autoref{fig:func-full}.
% , i.e. all three concretizations satisfy all the constraints listed in \autoref{fig:func-full}.
The scenes depicted in \autoref{fig:elab-same-sc} is semantically equivalent to the scene in \autoref{fig:scene}: in both cases, no \unk~relations are satisfied.
% neither scene satisfies any constraints that are not listed in \autoref{fig:func-full}.
Nevertheless, the position and relative heading of the actors greatly varies between the scenes.
In fact, each scene is placed in a different location on the map.
However, the scene depicted in \autoref{fig:elab-crooked} is not semantically equivalent to \autoref{fig:elab-same-sc} as it satisfies the \textcolor{blue1}{\qaCanSeePred{\actorBl}{\actorR}} relation, which originally evaluated to \unk~ (note that in our approach, the presence of \actorG~does not affect the visibility of \actorR, as discussed in \autoref{sec:elab-mapping}).
% Note that the depicted concretizations are only valid according to our proposed functional-to-logical constraint mapping: these scenes may be considered invalid if a different mapping is used (e.g. if said mapping defines a narrower field of view for the actors, such that \textcolor{blue1}{\qaCanSeePred{\actorG}{\actorBl}} no longer holds in \autoref{fig:elab-crooked} due to their relative headings).
\end{exline}


%%%%%%%%%%%%%%
AXIOMS
%%%%%%%%%%%%%
\newcommand{\axiom}[1]{\textit{#1}}
\begin{itemize}

    % \item%[\textit{C0}]
    % \err~\qaUnaryPred{Ax0}{o} \texttt{:=} \qaBinaryPred{rel}{o}{o}; where $\qa{rel} \in \Sigma\setminus\{\qaOnRoad\}$
    % \item[\axiom{Ax0}]
    % $\forall o \in \dslObjectSetI{P} \colon \interpretationFun{P}(c)(o, o) = 0$; where $\qa{rel} \in \Sigma\setminus\{\qaOnRoad\}$
    \item[\axiom{Ax0}]
    $\forall o \in \dslObjectSetI{P} \colon \neg \semantics{\qaBinaryPred{rel}{v}{v}}{P}{v \mapsto o}$; where $\qa{rel} \in \Sigma\setminus\{\qaOnRoad\}$
    
    
    $\forall o \in \dslObjectSetI{P} \colon \neg \semantics{\qaBinaryPred{rel}{v}{v}}{P}{v \mapsto o}$; where $\qa{rel} \in \Sigma\setminus\{\qaOnRoad\}$
    
    % \item%[\textit{C1}]
    % \err~\qaBinaryPred{Ax1}{$o_1$}{$o_2$} \texttt{:=} \qaBinaryPred{rel}{$o_1$}{$o_2$}, \texttt{!} \qaBinaryPred{rel}{$o_2$}{$o_1$}; where $\qa{rel} \in \symbolClass{R}{dist} \cup \{\qaNoColl\}$
    % \item[\axiom{Ax1}]
    % $\forall o_1, o_2 \in \dslObjectSetI{P} \colon \interpretationFun{P}(c)(o_1, o_2) = 1 \Rightarrow \interpretationFun{P}(c)(o_2, o_1) = 1 $; where $\qa{rel} \in \symbolClass{R}{dist} \cup \{\qaNoColl\}$
    \item[\axiom{Ax1}]
    $\forall o_1, o_2 \in \dslObjectSetI{P} \colon \semantics{\qaBinaryPred{rel}{v_1}{v_2}}{P}{v_1 \mapsto o_1, v_2 \mapsto o_2} \wedge \semantics{\qaBinaryPred{rel}{v_2}{v_1}}{P}{v_1 \mapsto o_1, v_2 \mapsto o_2}$; where $\qa{rel} \in \symbolClass{R}{dist} \cup \{\qaNoColl\}$


    % \item%[\textit{C2}]
    % \err~\qaBinaryPred{Ax2}{$o_1$}{$o_2$} \texttt{:=} \qaBinaryPred{r1}{$o_1$}{$o_2$},  \qaBinaryPred{r2}{$o_1$}{$o_2$}; where $\qa{r1} \in \symbolClass{R}{pos}, \qa{r2} \in \symbolClass{R}{pos}\setminus \qa{r1}$
    % \item[\axiom{Ax2}]
    % $\forall o_1, o_2 \in \dslObjectSetI{P} \colon \interpretationFun{P}(c_1)(o_1, o_2) = 1 \Rightarrow \forall c_2 \in \symbolClass{R}{dist}\setminus c_1 : \interpretationFun{P}(c_2)(o_1, o_2) = 0 $; where $\qa{r1} \in \symbolClass{R}{pos}, \qa{r2} \in \symbolClass{R}{pos}\setminus \qa{r1}$
    \item[\axiom{Ax2}]
    $\forall o_1, o_2 \in \dslObjectSetI{P} \colon \neg( \semantics{\qaBinaryPred{r1}{v_1}{v_2}}{P}{v_1 \mapsto o_1, v_2 \mapsto o_2} \wedge \semantics{\qaBinaryPred{r2}{v_1}{v_2}}{P}{v_1 \mapsto o_1, v_2 \mapsto o_2}) $; where $\qa{r1} \in \symbolClass{R}{pos}, \qa{r2} \in \symbolClass{R}{pos}\setminus \qa{r1}$
    
    % \item%[\textit{C3}]
    % \err~\qaBinaryPred{Ax2}{$o_1$}{$o_2$} \texttt{:=} \qaBinaryPred{r1}{$o_1$}{$o_2$},  \qaBinaryPred{r2}{$o_1$}{$o_2$}; where $\qa{r1} \in \symbolClass{R}{dist}, \qa{r2} \in \symbolClass{R}{dist}\setminus \qa{r1}$
    % \item[\axiom{Ax3}]
    % $\forall o_1, o_2 \in \dslObjectSetI{P} : \forall c_1 \in \symbolClass{R}{dist} : \interpretationFun{P}(c_1)(o_1, o_2) = 1 \Rightarrow \forall c_2 \in \symbolClass{R}{dist}\setminus c_1 : \interpretationFun{P}(c_2)(o_1, o_2) = 0 $
    \item[\axiom{Ax3}]
    $\forall o_1, o_2 \in \dslObjectSetI{P} \colon \neg( \semantics{\qaBinaryPred{r1}{v_1}{v_2}}{P}{v_1 \mapsto o_1, v_2 \mapsto o_2} \wedge \semantics{\qaBinaryPred{r2}{v_1}{v_2}}{P}{v_1 \mapsto o_1, v_2 \mapsto o_2}) $; where $\qa{r1} \in \symbolClass{R}{dist}, \qa{r2} \in \symbolClass{R}{dist}\setminus \qa{r1}$
\end{itemize}


%%%%%%%%%%%%%%%%%%%
DETAILS ABOUT SCENIC
%%%%%%%%%%%%%%%%%%%

\subsection{Existing restrictions over scene specifications}
\label{sec:pre-restrictions}

% \todo{scenic is a subset of my proposed semantics}
Functional scene specifications as defined in \autoref{sec:pre-lang} cannot be handled by the current state-of-the-art in terms of traffic scene concretization, namely the \scenic~tool \cite{Fremont2019ScenicLanguage}, which uses a probabilistic programming language as input for a sampling-based concretization approach.

% (i.e. approaches that can concretize any traffic scene, rather than scenes from a specific category).
% \scenic~is a framework that uses a probabilistic programming language for functional-level scene specification.
% The framework also includes a  scene concretization approach based on rejection sampling.


% \todo{"Oszkar, please check formalization"}
% In \scenic, the sample space for each variable in the scene specification (e.g the position and heading of each actor) must be defined at instantiation-time.
% The default sample space for an actor may be restricted through \textit{a single} positional relation (constraint), optionally accompanied by a distance relation, applied with respect to another instantiated actor.
% For a given partial model defined over an object set $\dslObjectSet$, this implies that an object $o_1 \in \dslObjectSet$ cannot be the target of more than one positional relation.


Additionally, \scenic~does not use an underlying PM rep for scenes, thus it cannot detect errors

At the level of partial models, this corresponds to relaxing certain positive constraints (i.e. setting their truth value to \unk).
This constraint is formalized as follows: 
% \err~\qaTernaryPred{AxScenic}{$o_1$}{$o_2$}{$o_3$} \texttt{:=} \qaBinaryPred{r1}{$o_2$}{$o_1$},  \qaBinaryPred{r2}{$o_3$}{$o_1$}, $o_2 \neq o_3$; where $\qa{r1}, \qa{r2} \in \symbolClass{R}{pos}$
% $\forall o_1, o_2, o_3 \in \dslObjectSetI{P} : \neg (\interpretationFun{P}(r1)(o_2, o_1) = 1 \wedge \interpretationFun{P}(c_1)(o_3, o_1) = 1 \wedge o_2 \neq o_3 )$, where $\qa{r1}, \qa{r2} \in \symbolClass{R}{pos}$.
$\forall o_1, o_2, o_3 \in \dslObjectSetI{P} \colon \neg (\semantics{\qaBinaryPred{r1}{v_2}{v_1}}{P}{v_1 \mapsto o_1, v_2 \mapsto o_2} \wedge \semantics{\qaBinaryPred{r2}{v_3}{v_1}}{P}{v_1 \mapsto o_1, v_3 \mapsto o_3} \wedge o_2 \neq o_3 )$, where $\qa{r1}, \qa{r2} \in \symbolClass{R}{pos}$.
A consequence of this additional requirement is that cyclic positional relations, including undirected cycles, are not handled natively by \scenic. 

\begin{exline}
Considering these restrictions, \autoref{fig:func-scenic} presents a \scenic-expressible subset of the relations included in \autoref{fig:func-full}.
Among the 6 possible positional relations defined over a pair of actors, at most 2 may be expressed by \scenic.
Note that the order of actor definitions influences the relations that may be possibly included.
In this example, actors are defined in the following order: \actorG, \actorBl, then \actorR.
Considering this ordering, \textcolor{OliveGreen}{\qaRightPred{\actorG}{\actorR}} may have been included instead of \textcolor{OliveGreen}{\qaLeftPred{\actorBl}{\actorR}}.
\end{exline}


%%%%%%%%%%%%%%%%
\subsection{Restrictions of the \scenic~\fss~language}
\label{sec:pre-restrictions}

Due to limitations of the underlying scene concretization approach of \scenic, actors may only be the target of at most one positional relation.
Formally, this corresponds to applying the following rule:
{\footnotesize\infer
{\interpretationFun{P}(\qa{r2})(c, a) = \interpretationFun{P}(\qa{r2})(c, a) \oplus \false}
{a, b, c \in \dslObjectSetI{P} \wedge
b \neq c \wedge
\interpretationFun{P}(\qa{r1})(b, a) = \true }}
, where $\qa{r1}, \qa{r2} \in \symbolClass{R}{pos}$.
This states that if there exists a positional relation $r1$ that targets $a$, all other positional relations $r2$ that target $a$ are known to be \false.

A consequence of this additional rule is that \scenic~would falsely flag cyclic positional relation structures (including undirected cycles) as \err{}s.
In fact, since \scenic~does not use an underlying partial model to represent scenes, it is incapable of expressing such structures through its input language, despite their satisfiability in the context of scene concretization.

\todo{havnt yet reviewed the example}
\begin{exline}
Considering these restrictions, \autoref{fig:func-scenic} presents a \scenic-expressible subset of the relations included in \autoref{fig:func-full}.
Among the 6 possible positional relations defined over a pair of actors, at most 2 may be expressed by \scenic.
Note that the order of actor definitions influences the relations that may be possibly included.
In this example, actors are defined in the following order: \actorG, \actorBl, then \actorR.
Considering this ordering, \textcolor{OliveGreen}{\qaRightPred{\actorG}{\actorR}} may have been included instead of \textcolor{OliveGreen}{\qaLeftPred{\actorBl}{\actorR}}.
\end{exline}


%%%%%%%%%%%%%%%%%%%%
Logical Scene
%%%%%%%%%%%%%%%%%%%%
% \todo[color=Yellow]{lightweight formalization, atomic predicates over terms. And then the logical problem is comprised of numeric constraints. The relation is a mapping. And then we say what the solution is, basically value given to each variable}
% \todo{rewrite this. will be significantly reduced once above if formalized}
% A functional scene specification represented by a partial model corresponds to an abstract scene concretization problem, which must first be mapped to a corresponding numeric (logical-level) problem.
% In fact, each symbol in the abstract vocabulary $\Sigma$ corresponds to a logical (numeric) constraint over formally represented actors.
% For each relation in the partial model that evaluates to \true, the corresponding numeric constraint is added to the numeric problem.
% Similarly, for \false~relations, the negation of the corresponding numeric constraint is included.
% Numeric  constraints for \unk~relations are excluded from the numeric problem.
% A solution to the logical-level numeric problem, i.e. a concrete scene, corresponds to an assignment of the numeric variables that define each actor st. all the included numeric constraints are satisfied.














mention about if numeric constraint corresponding to abstract relation is satisfied, the the correspoding abstract relation is also satisfied (CORRECTNESSS (SOUNDNESS) Claim.








% Each relation in the partial model is mapped derived according to mapping between the \textit{relation symbols} in $\Sigma$ and  that must be satisfied by the derived concrete model.
% The collection of these numeric constraints forms the logical-level numeric problem.
% As such, each relation in the partial model is mapped to a numeric constraint
% The abstract concretization problem defined at the functional level is mapped to a corresponding numeric problem at the logical level.
% Each relation symbol in $\Sigma$ corresponds to a numeric constraint evaluated over the variables associated to each actor. 

% \todo[color=red]{go through abstract relations, each 0 or 1 edge is mapped to a numeric solution. Solution is assignment of values to numerical values which satisfy the constraints.}
% \todo{basically, a concrete model must satif=sfy all the 1 constraints, and may satusfy the 1/2 constraints. As such, the 1/2 constraints will be refined to 1 or 0. This is done based on the concrete numeric values}

%%%%%%%%LOGICAL-TO-CONCRETE%%%%%%%%

% Once a logical scene containing numeric constraints is created, a decision procedure is required to obtain a concrete scenes.
% Such numeric problems may be handled by various approaches such as SMT solver \cite{} or CSP solver \cite{}.
% However, most existing approaches are not customized for the domain of traffic scene concretization.
% One existing approach \cite{abdessalem} leverages a genetic algorithm to generate test cases based on a restricted modeling space that does not consider functional-level scene specifications.
% Otherwise, the \scenic~tool \cite{scenic} handles functional constraints through an approach based on based on rejection sampling.
% However, the input language is subject to certain structural limitations, as discussed in \autoref{sec:elab-structure}.

% A possible scene concretization is shown in \autoref{fig:sceneAbsLevels}.
% Note that the derived numeric values for the scene variables do not provide a unique solution: for example, the $\paramR{h}$ variable may take any value in the concretization at it is not subject to any numeric constraints at the logical level.

\todo{could we entirely remove this example?}
\begin{exline}
% The scene description\autoref{fig:sceneAbsLevels} represents a 
% A  functional-level scene specification, as well as the visualization of a corresponding concrete scene, 
% The scene contains two  both of which are \car{}s.
% Note that the variables corresponding to each actor are colored according to the vehicle they represent, as shown in the visualisation.
% The scene contains two abstract constraints, namely \textcolor{OliveGreen}{\qaFrontPred{\actorR}{\actorBl}} and
% \textcolor{LimeGreen}{\qaMedPred{\actorBl}{\actorR}}, both of which are shown as arrows in the visualization.
% Note that although no positional constraint is specified between \actorR~and \actorBl, the \qaBehindPred{\actorR}{\actorBl} constraints holds in the visualised concrete scene, as allowed by the open-world assumption.

% A logical scene and a corresponding functional scene are shown in \autoref{fig:sceneAbsLevels}, where the numeric actor representations exclude width and length values, for simplicity.

The concretization problem presented in \autoref{fig:sceneAbsLevels} is defined over two \qaCar~actors \actorR~and \actorBl.
The variables corresponding to each actor are colored according to the vehicle they represent, as shown in the included visualisation.
The numeric actor representations used at the logical and concrete levels exclude width and length variables, for simplicity.

The problem consists of three functional relations: two positive relations \textcolor{OliveGreen}{\qaFrontPred{\actorR}{\actorBl}} and \textcolor{LimeGreen}{\qaMedPred{\actorBl}{\actorR}} (visualised as arrows), and a negated relation 
\texttt{!}\qaRightPred{\actorBl}{\actorR}, which are mapped to corresponding numeric constraints depicted using the same color.
% the
% \textcolor{OliveGreen}{$\exists r > 0: \paramBl{x} = \paramR{x} + r \cos{\paramR{h}} \wedge \paramBl{y} = \paramR{y} + r \sin{\paramR{h}}$},
% \textcolor{LimeGreen}{$c_l \leq \sqrt{(\paramR{x} + \paramBl{x})^2 + (\paramR{y} + \paramBl{y})^2} \leq c_u$}
% and 
% $\neg \Big( \exists r > 0: \genfrac{}{}{0pt}{}{\paramR{x} = \paramBl{x} + r \cos{(\paramBl{h} - \sfrac{\pi}{2})} \wedge}{\paramR{y} = \paramBl{y} + r \sin{(\paramBl{h} - \sfrac{\pi}{2})}} \Big)$
% logical constraints respectively.
% \todo[color=Yellow]{below is more appropriate here}

The mapping between functional and logical problems is not unique as it varies between concretization approaches.
% The former is mapped according to the mapping proposed in \cite{scenic}, whereas the latter conforms to the mapping proposed in \autoref{sec:elab-mapping}.
In this example, the numeric equivalent constraint of \textcolor{OliveGreen}{\qaFrontPred{\actorR}{\actorBl}} states that the center point of \actorBl~must be placed at an angle $\paramR{h}$ (i.e. exactly ahead) from the center point of \actorR.
Similarly, \texttt{!}\qaRightPred{\actorBl}{\actorR} states that \actorR~must not be placed at a $- \sfrac{\pi}{2}$ angle (i.e. to the right) measured from $\paramB{h}$ wrt. the center point of \actorR.
Finally, the \textcolor{LimeGreen}{\qaMedPred{\actorBl}{\actorR}} constraints capture that the Euclidean distance between the center points of \actorBl~and \actorR~must be between $c_l$ and $c_u$, which are constant lower and upper bound values.

The concrete scene is defined as an assignment of actor variables such that  \textcolor{OliveGreen}{\qaFrontPred{\actorR}{\actorBl}}, \textcolor{LimeGreen}{\qaMedPred{\actorBl}{\actorR}} and \texttt{!}\qaRightPred{\actorBl}{\actorR} are satisfied.
Note that the derived numeric values do not provide a unique solution: for instance, the $\paramBl{h}$ variable may take any value except $0$ in order to satisfy all the constraints.
% \todo{explain what each numeric constraint means}
\end{exline}



%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we will discuss the current state-of-the-art in terms of concretizing functional AV test scenes, namely the \scenic \cite{Scenic} tool.
% \todo{does this apply to other languages too? wld be cool to generalize the state-of-the-art}
% Specifically, we will discuss the underlying decision procedure used by \scenic, as well as the adaptability of the constraints detailed in \autoref{sec:pre-lang} to the particular constraint structure handled by the tool.
% This sections only provides a high-level overview of the relevant components of \scenic.
% You may refer to the original paper for more thorough details about the syntax and the mathematical semantics of the \scenic specification language.


% \subsection{Multi-Objective Search}




% \todo{comment about logical-level distance, mybe remove from figure}

% is defined at the scene specification level 
% Sample space my be limited by a constraint over dynamic components introduced at definition-time.
% Such constraints may be at logical level (e.g \actorG \tptpStyle{= Car in CircularRegion(center=} \actorR \tptpStyle{, radius=30}) or at the functional level
% (e.g \actorBl \tptpStyle{ = Car left of } \actorG).
% In the latter case, an functional-to-logical constraint mapping is used to represent the constraints in the sample-space domain.

% The expressiveness of constraints applied to dynamic actors at definition-time is limited.
% Specifically, such constraints can only represent a tree structure, as the sample space of a certain dynamic element may only be limited according to constraints applied over existing actors.
% As such, definition-time constraints are local wrt. the defined dynamic element.
% Nevertheless, \scenic does handle global constraints, applied over all defined dynamic elements.
% However, these constraints do not influence the rejection sampling approach used for scene concretization: their satisfiability is only checked after sampling, as acceptance criteria for the derived sample.


% \subsection{General Overview of the workflow}

% \begin{itemize}
%     \item Given an abstract Scene specification
%     \item Initialize the actors
%     \item Give positions to each actor at each iteration of NSGA
%     \item Evaluate fitness, which relates to the constraints for the specific Scene specification under test
%     \item Repeat until end condition is met (mention the end condition)
% \end{itemize}

% \subsection{Additional Tooling}

% \begin{itemize}
%     \item Simulator integration
%     \item Output images
% \end{itemize}



%%%%%%%%%%%%%%%%
MOO integration, old text
%%%%%%%%%%%%%%%%


% In this paper, given a functional scene specification as input, each numeric constraint derived from an included functional relation corresponds to a testing requirement.
% For each requirement, a distance function $DF_i$ is defined such that $DF_i = 0$ iff the requirement holds (i.e. the corresponding numeric constraint, and thus the functional relation, holds for a given candidate solution).
% Otherwise, the distance value is computed according to \autoref{fig:distance-functions}.


% (i.e. the corresponding numeric constraint, and thus the functional relation, holds for a given candidate solution).
% Otherwise, the distance value is computed according to \autoref{fig:distance-functions}.

% (which may be covers a collection of numeric constraints, categorized by the type of the corresponding functional relation.
% Considering that the number of functional relation types may be extended according to specific traffic scene requirements, we 
% In this paper, we proposed 5 categories of functional relations (and corresponding numeric constraints), as listed in \autoref{sec:func-lang} We propose an approach where functional relations 


% Specifically, each numeric constraint is first transformed into a soft constraint, which allows for we define one objective function per type of functional relation that a concrete scene must comply with.
% We have introduced five functional relation types in \autoref{sec:func-lang}


% For that purpose, we define custom \textit{distance functions} applied over numeric constraints to determine how far a candidate solution is from satisfying the testing requirements.

% At every iteration, NSGA derives a candidate solution.
% The distance is measured
% If distance is 0, then it is a solution.

\begin{comment}
% and incorporates custom objective functions applied over numeric constraints.
% \autoref{fig:distance-functions} defines objective functions $OF_{i}$ for each relation.
% If a functional relation holds  (i.e. evaluates to \textsc{True}), then $OF_{i}$ evaluates to 0. Otherwise, we assign a (positive) numeric value representing the amount of error. As such,  the closer the $OF_{i}$ value is to 0, the closer is the concretization to satisfy the corresponding functional relation.
% % , it signifies that the corresponding functional constraint holds (i.e. evaluates to \textsc{True}). 
% %$OF_{i}$ may only evaluate to positive values, such that an optimal solution has all $OF_{i}$ values equal to 0.
% %In fact, the closer the $OF_{i}$ value is to 0, the closer is the concretization to satisfy the corresponding functional constraint.
% Unlike in Scenic, this allows graceful degradation for our scene concretization approach: even if some functional relations are not satisfied, our approach will provide an approximately satisfactory solution.
% %where most constraints  the if our approach is incapable of finding a concretization that satisfies all input constraints, it may find a solution that satisfies most constraints, or does not violate the constraints badly.
% % \todo{Graceful degredation: we satisfy most, or we do not violate them badly}
% % \todo{if value is very low, we are close to a solution. This is related to below}

%%%%%%%%%%%%% EPSILON ISSUESSS
% \todo{ASK DANIEL how we can use real values in objective functions. How epsilon behaves. Potential solution is just to write epsilon instead of 0 above}
% Our proposed objective functions return floating point values.
% \todo{double negation}
% However, our \moopt~approach is not susceptible to asymptotic behavior (i.e subsequent iterations get close to an optimal solution without ever reaching it) because the satisfaction of a constraint does not rely on the positioning of an actor on an infinitesimal area (i.e. the solution space for the concretization problem are non-infintesimal, as discussed in \autoref{sec:elab-mapping}).

% \autoref{fig:distance-functions} explicitly return 0 when the corresponding numeric condition is met.
% \todo{Also, we should mention that even tho we are using floats, we still do not measure with epsilon, becausethe OFs (fig 6) include a region, so multiple correct answers. e are always explicitly givin back 0 for successes. But maybe this causes an issue considering that we have a bunch of lessThanOrEqualToos in fig 4. This is avoided by the "if" strctures in fig 6. Make this "if structure" explicit for dist|canSee|onRoad}
\end{comment}

%%%%%%%%%%%%%
Objective functions
%%%%%%%%%%%%%

% \textit{Distance and objective functions}:
\todo{improve wording}
\textit{Objective functions}:
In our approach, an objective function is defined for each type (category) of functional relations, as listed in \autoref{fig:distance-functions}.
A fitness value that considers all the corresponding objective function returns a fitness value that considers all functional relations of that type in the partial model  
%(i.e. for each relation symbol in $\Sigma$).
For our five types of functional relations, the respective distance functions are listed in \autoref{fig:distance-functions}.
Each relation symbol of a specific type is handled similarly. 
%Note that relation types may collect multiple relation symbols that are treated similarly (i.e. in the case of \textbf{positional} and \textbf{distance} relations).
 
 
 
 
%%%%%% AGGREGATE OBJECTIVE FUNCTIONS
% \todo{improve wording}
% During design-space exploration, we evaluate the fitness of a population through five objective functions $OF_{j\in[1, 5]}$ that aggregate the distance functions for all constraint instances of a given type.
% \textit{Objective functions}:
After evaluating the distance functions over $CS$, we aggregate the values of constraints associated to the same relation type into a single objective function.
As such, our approach will yield, in this case, 5 (aggregate) objective functions.
% , one for each type of relation. 
% For instance, the distance function values of all positional constraints included in a numeric problem are summarized into a single objective function. % evaluated over a candidate solution.

This allows for weighting of distance functions (e.g. handling of hard and soft constraints) according to relation types, which is particularly useful if a solution cannot be derived.
For instance, to increase realisticness of approximate solutions, we may prioritise \textbf{road placement} and \textbf{collision avoidance} constraints.
\todo{might need more here}

% \todo{formalization isintentionally complex. This is how }
% \todo[color=Yellow]{discuss that weight function is applied to the collection of constraints of a given type}

Formally, given a set $\constrSetI{N}$ of numeric constraints, an objective function (for a given relation type $T$) is formalized as follows:
% \todo{in reality, we are single-objctive cuz we only accept all-0 objective functionn values}
% \todo{improve formalization}

% \todo[color=Yellow]{Each constraint is an objective No need to change current formalization of OF. we are optimizing each constraint/objective, but we are optiizing them together, according to the formalization. So the formalization is just a technique to summarize the objectives. DF bvecomes OF, objective function. OF becomes aggregated objective function}
% {\footnotesize
% \[
% OF_i(cons, \mathbf{C}) = f\left(\sum_{\begin{tabular}c \in cons\\c is type \end{tabular}} OF_i(c, \mathbf{C}) \llbracket type_i (c) \rrbracket\right)
% \]
% }

{\footnotesize
\[
OF_{T} = f_{T}\left(\sum_{\makecell[c]{ c \in \constrSetI{N},\\c.type \texttt{ = } T}} DF_{id(T)}(c)% \llbracket type_i (c) \rrbracket
\right)
\]
}, where

\begin{itemize}
    \item $f_{T}()$ is a positive, non-decreasing weight function \todo{enough? We basically need the 0 to stay the same place},
    \item $id(T) \in [1, 5]$ denotes the distance function id associated to $T$, as used in \autoref{fig:distance-functions}, and 
    \item $DF_{id(T)}(c)$ is the outcome of a distance function measured over a single constraint $c$.
    % \item $type_i(c)$ is a condition that returns \textit{true} if $c$ is of the type corresponding to $i$ (e.g. $type_1(c)$ returns \textit{true} if $c$ is a positional constraint). 
\end{itemize} 
 
 
 
 
Considering that the number of functional relation symbols of a given scene concretization problem may be extended by experts, the number of required objective functions for an arbitrary scene specification is not defined a priori.
As such, we propose a \mom~problem formalization that can address an arbitrary number of objective functions.

==> chp/syntax.tex <==
% \todo[inline,color=red]{Below is redundant}

% % \todo[color=yellow,inline]{Vnum does not parametrized with P. What about $\langle\mathcal{O}_P,\mathcal{I}_P,\mathcal{V}_P\rangle$, so they have the same formatting?} 
% % \todo{Would it be possible to divide $Obj_P$ into $Obj_{str}$ and $Obj_{num}$. This would make section 4.2 easier.}
%  and is the existential interpretation of each predicate symbol in $\Sigma$ using 3-valued logic. 
% $\interpretationNumFun{P}$ is the numerical interpretation of $\symbolClass{TN}{i}$ instances in $\Sigma$. It is only a partial interpretation on $\Sigma$.
% An object $n$ in $\dslObjectSetI{P}$ is \emph{Bound} to a specific value if $\interpretationNumFun{P}(n) \neq \unbound$. 
% Otherwise, the $n$ is \emph{Unbound}.
% % \todo[color=yellow]{what about $\ast$ instead of $\nexists$? Because $\ast$ can can surely exist}
% \begin{itemize}

%     \item $\interpretationDef{P}{\symbolClass{T}{i}}{\dslObjectSetI{P}}{\{1, 0, \sfrac{1}{2}\}}$ as in ICSE 2018.
%     \item $\interpretationFun{P} : \symbolClass{c}{j} \rightarrow{} \dslObjectSetI{P}$ as in FASE 2020.
%     % \item $\mathcal{I}_P(N_k): \dslObjectSetI{P} \rightarrow{} (\{1, 0, \sfrac{1}{2}\}, \{0, 1\})$ . 
    
%     % \item $\interpretationDef{P}{\symbolClass{N}{i}}{\dslObjectSetI{P}}{\{1, 0, \sfrac{1}{2}\}}$, similar to $\symbolClass{C}{j}$. 
%     % \item $\interpretationDef{P}{\symbolClass{N}{r}}{\dslObjectSetI{P}}{\{1, 0, \sfrac{1}{2}\}}$, similar to $\symbolClass{C}{j}$.
%     % \begin{itemize}
%     %     \item The first tuple element defines whether it is true, false or unspecified if an object is an instance of $N_k$.
%     %     \item The second tuple element defines whether it is false or true that a numeric value is associated to the object.
%     % \end{itemize} 
%     % \todo{Should we combine the last two tuple elements?}
%     \item $\interpretationDef{P}{\symbolRef{R}{k}}{\dslObjectSetI{P} \times \dslObjectSetI{P}}{\{1, 0, \sfrac{1}{2}\}}$ as in ICSE 2018.
    
%     \item $\interpretationDef{P}{\symbolRef{H}{l}}{\dslObjectSetI{P} \times \ldots \times \dslObjectSetI{P}}{\{1, 0, \sfrac{1}{2}\}}$, defined in \autoref{sec: HE+Check}.
    
%     \item $\interpretationDef{P}{\dslExistSymbol}{\dslObjectSetI{P}}{\{1, 0, \sfrac{1}{2}\}}$ as in ICSE 2018.
    
%     \item $\interpretationDef{P}{\dslEqualSymbol}{\dslObjectSetI{P} \times \dslObjectSetI{P}}{\{1, 0, \sfrac{1}{2}\}}$ as in ICSE 2018.
    
%     % \item $\mathcal{V}_{num}(N_k): \{n | n \in \dslObjectSetI{P} \wedge \mathcal{I}_P(n)[1] = 1)\} \rightarrow{} \{\mathbb{R}, \nexists\}$
    
%     \item $\interpretationNumDef{P}{\symbolClass{TN}{i}}{\dslObjectSetI{P}}{\mathbb{R} \cup \{\unbound\}}$

%     % \item $\interpretationNumDef{P}{\Sigma \char`\\ \symbolClass{T}{i}} {\dslObjectSetI{P}}{\unbound}$
% \end{itemize}
%     % \item Numeric types are gathered in a set $Obj_{num} \subset Obj_P$. To define $Obj_{num}$, we simply query $Obj_P$ for all objects that is must-labeled with a numeric type (ex. any object in $P$ such that $type_{int}(P) = 1$.)
    
%     % $\mathcal{A}_P$ is the set of all numerical attributes in partial model $P$ \todo[color=yellow]{arent they objects?} (regardless of the value \{ 0, 1/2, 1\} of its parent object), and $\mathcal{V}_P$ is the interpretation of $\mathcal{A}_P$. 
%     % \textbf{Each element in $\mathcal{V}_P$ is interpreted as the domain of numeric values} that are valid with respect to constraints applied on $P$.
%     % Initially, these domains may be $\mathbb{R}$ or $\mathbb{Z}$ according to the type of the attribute.
%     % \item NEW: \todo[inline]{For model generation purposes, each element in $\mathcal{A}_P$ may be considered as a graph node with a specific type (Int, Float, ...) that is associated to its container class by a reference. 
%     % We assume that attribute multiplicity is always exactly 1, therefore, the existence of attributes does not affect decision rules.}
%     % \todo[color=yellow]{find, neg, or, and from sec 4.1, including example. SYNTAX: diffictulty is defining implicit variables within a body. Implicit exists for most cases, but might be forall for neg find}
%     % \todo[color=yellow]{Add hyperedge to Sigma, use it for check (replace eval)}
%     % \todo[color=yellow]{Seperate logic part from pattern structural part}
%     % \todo[color=yellow]{make seperate section for check expression}

% \subsection{Hyperedges and Attribute Expressions}
% \label{sec: HE+Check}

% \todo[inline]{Do we really need this? Are the Syntax and Semantics tables not sufficient?}

% There is a hyperedge among a set of variables \texttt{\{$p_1$, $p_2$, ..., $p_m$\}} if and only if there exists a constraint $con(v_1, v_2, ..., v_m)$ := $con _{str}(v_1, v_2, ..., v_m, a_1, a_2, ..., a_m) \wedge con _{num}(a_1, a_2, ..., a_m)$ such that $con _{str}(v_1, v_2, ..., v_m, a_1, a_2, ..., a_m)$ is satisfied and $\forall i \in [1, m] \cap \mathbb{N}, p_i \mapsto a_i \mapsto w_i$ where $w_i$ is a variable of object $o_i$ mapped to by $v_i$.  \todo[inline,color=red]{above is redundant}

% % \todo[inline]{Need to modify this!!}

% \begin{table*}[h]
%     \centering
%     \begin{tabular}{r@{ }r@{ }c|c|l}
    
%     & & Math. Syntax & Check Syntax & \\
    
%     \hline
%     \multicolumn{5}{|c|}{Pattern Structure Part}\\
%     \hline
    
%     % && \hl{We can probably rename the "body" predicate}&\hl{Distinguish terminal from non-terminal symbols beter}&\\
%     % \hl{ex in Type check, C is not an arbitrary string, rather a specific class name}&\\
    
%     $\nonTerminal{\varphi}$ & $\vcentcolon=$ &
%     $Q(\nonTerminal{params}) \Leftrightarrow{} \nonTerminal{bodies}$ \hl{negate?}&
%     $\nonTerminal{annotation} \checkStyle{pattern} \nonTerminal{name} $ & 
%     \emph{pattern defn} \\
%     &&&$\checkStyle{(} \nonTerminal{params} \checkStyle{)} \nonTerminal{bodies}$&\\
    
%     %hline
    
%     $\nonTerminal{params}$ & $\vcentcolon=$ &
%     $\nonTerminal{param}$ & 
%     $\nonTerminal{param}$ & 
%     \emph{parameter} \\
%     & $|$ & 
%     $\nonTerminal{params}, \nonTerminal{param}$ & 
%     $\nonTerminal{params}\checkStyle{, } \nonTerminal{param}$
%     & \emph{parameter set} \\
    
%     %hline
    
%     $\nonTerminal{param}$ & $\vcentcolon=$ &
%     $v$ & 
%     $v$ & 
%     \emph{variable} \\
%     & $|$ & 
%     $\termClass{T}{v}$ \hl{add this in semantics for structural part?}& 
%     $v \checkStyle{ : } \nonTerminal{\symbolClass{EClassifier}{}}$
%     & \emph{typed variable} \\
    
%     %hline
    
%     $\nonTerminal{bodies}$ & $\vcentcolon=$ &
%     $\exists \nonTerminal{params} : \nonTerminal{body}$ & 
%     $\checkStyle{\{} \nonTerminal{body} \checkStyle{\}}$ 
%     & \emph{constraint} \\
%     & $|$ & 
%     $\exists \nonTerminal{params} : \nonTerminal{body} \:\vee \nonTerminal{bodies}$ & 
%     $\checkStyle{\{} \nonTerminal{body} \checkStyle{\} or } \nonTerminal{bodies} $ &
%     \emph{constraint sequence} \\
    
%     %hline
    
%     $\nonTerminal{body}$ & $\vcentcolon=$ &
%     $\nonTerminal{constr}$ & 
%     $ \nonTerminal{constr} \checkStyle{;}$ &
%     \emph{constraint body} \\
%     & $|$ & 
%     $ \nonTerminal{constr} \wedge \nonTerminal{body}$ & 
%     $\nonTerminal{constr} \checkStyle{;} \: \nonTerminal{body}$ &
%     \emph{disj. of constrain bodies} \\
    
%     %hline
    
%     $\nonTerminal{constr}$ & $\vcentcolon=$ & 
%     $\nonTerminal{StrConstr} | \nonTerminal{NumConstr}$ & 
%     $\nonTerminal{StrConstr} | \nonTerminal{NumConstr}$ & 
%     \emph{constraint types} \\
    
%     %hline
    
%     $\nonTerminal{StrConstr}$ & 
%     $\vcentcolon=$ & $\termClass{T}{\nonTerminal{p}}$ & 
%     $\nonTerminal{\symbolClass{T}{}} \checkStyle{(} \nonTerminal{p}\checkStyle{)}$ & \emph{type check} \\
%     % & $|$ & $\termClass{N}{p}$ & \checkStyle{java N(p)} & \emph{primitive type check} \\
%     & $|$ & 
%     $\termReference{R}{\nonTerminal{p_1}}{\nonTerminal{p_2}}$ &
%     $\nonTerminal{\symbolClass{TC}{}} \checkStyle{.} \nonTerminal{\symbolClass{R}{}}    \checkStyle{(}\nonTerminal{p_1}\checkStyle{, }\nonTerminal{p_2}\checkStyle{)}$ &
%     \emph{reference and attribute check}\\
    
%     &&\hl{ref/attr navig missing}&&\\
% %    & $|$ & $\termClass{C}{p_1} \wedge \termReferenceInd{R}{p_1}{p_2}{1} \wedge \termReferenceInd{R}{p_2}{p_3}{2} \wedge \ldots \wedge \termReferenceInd{R}{p_n}{p_{n+1}}{n}$ & $\checkStyle{C.R1.R2. ... .Rn(}$\nonTerminal{p_1}$\checkStyle{, p(n+1))}$ & \emph{reference and attribute navigation}\\
%     & $|$ & 
%     $\termTCReference{R}{\nonTerminal{p_1}}{\nonTerminal{p_2}}$ &
%     $\nonTerminal{\symbolClass{TC}{}} \checkStyle{.} \nonTerminal{\symbolClass{R}{}}   \checkStyle{+(}\nonTerminal{p_1}\checkStyle{, }\nonTerminal{p_2}\checkStyle{)}$ &
%     \emph{ref and attr transitive closure}\\
    
%     & $|$ & $\nonTerminal{p_1} \dslEqualSymbol \nonTerminal{p_2} \: | \: \neg (\nonTerminal{p_1} \dslEqualSymbol \nonTerminal{p_2})$& \checkStyle{}$\nonTerminal{p_1}$\checkStyle{ == }$\nonTerminal{p_2}$\checkStyle{} | \checkStyle{}$\nonTerminal{p_1}$\checkStyle{ != }$\nonTerminal{p_2}$\checkStyle{} & \emph{equivalence/inequivalence}\\
%     % & $|$ & $\neg (p_1 \dslEqualSymbol p_2)$ & \checkStyle{}$\nonTerminal{p_1}$\checkStyle{ != }$\nonTerminal{p_1}$\checkStyle{} & \emph{inequivalence}\\

%     & $|$ & 
%     $Q(\nonTerminal{binding})$ & 
%     $\checkStyle{find} \nonTerminal{Q} \checkStyle{(} \nonTerminal{binding} \checkStyle{)}$ \hl{unsure} & 
%     \emph{pattern match}\\
%     & $|$ & 
%     $\forall \: \nonTerminal{binding} :\neg Q(\nonTerminal{binding})$ & 
%     $\checkStyle{neg find} \nonTerminal{Q} \checkStyle{(} \nonTerminal{binding} \checkStyle{)}$ & 
%     \emph{negated pattern match} \\
%     & $|$ & 
%     $Q^+(\nonTerminal{p_1}, \nonTerminal{p_2})$ & 
%     $\checkStyle{find} \nonTerminal{Q} \checkStyle{+(} \nonTerminal{bind_v} \checkStyle{)}$ & 
%     \emph{pattern transitive closure}\\

%     & $|$ & 
%     $(\nonTerminal{constr_1} \wedge \nonTerminal{constr_2}) \vee $ & 
%     $\nonTerminal{constr_1}\checkStyle{?} \nonTerminal{constr_2} \checkStyle{:} \nonTerminal{constr_3}$ & 
%     \emph{ternary operation} \\
%     && $(\neg \nonTerminal{constr_1} \wedge \nonTerminal{constr_3})$&&\\
    
%     %hline
    
%     % & $|$ & $body_1 \wedge body_2$ &  $\nonTerminal{body1}$ \checkStyle{;} $\nonTerminal{body2}$ \checkStyle{;} & \emph{constraint conjunction} \\
%     $\nonTerminal{binding}$ & $\vcentcolon=$ &
%     $\nonTerminal{p}$ & 
%     $\nonTerminal{p}$ & 
%     \emph{parameter} \\
%     & $|$ & 
%     $\nonTerminal{p}, \nonTerminal{binding}$ & 
%     $\nonTerminal{p}\checkStyle{, } \nonTerminal{binding}$
%     & \emph{parameter set} \\
    
%     %hline
    
%     $\nonTerminal{p_n}$ & $\vcentcolon=$ & 
%     $c$ & 
%     $\nonTerminal{\symbolClass{c}{}}$ & 
%     \emph{metamodel literal}\\
%     & $|$ & 
%     $v$ & 
%     $v$ & 
%     \emph{variable}\\
    
%     %hline
    
%     $\nonTerminal{annotation}$ & $\vcentcolon=$ &
%     & $\checkStyle{@Constraint} | \checkStyle{@QueryBasedFeature} | \epsilon$ & \emph{annotation defn} \\
%     %hline
%     $\nonTerminal{name}$ & $\vcentcolon=$ &
%     & $\emph{EString}$ & \emph{name defn} \\
    
%     \hline
%     \multicolumn{5}{|c|}{Logical Evaluation of Check Expression}\\
%     \hline
    
%     $\nonTerminal{NumConstr}$ & $\vcentcolon=$ &
%     $\termClass{H}{binding} \Leftrightarrow{} \nonTerminal{eqn} $ & 
%     $\checkStyle{check(} \nonTerminal{eqn} \checkStyle{)}$ & 
%     \emph{predicate evaluation} \\
%     %hline
%     $\nonTerminal{eqn}$ & $\vcentcolon=$ &
%     $\nonTerminal{op}(\nonTerminal{X_1}, \nonTerminal{X_2})$ & 
%     $\nonTerminal{X1} \nonTerminal{op} \nonTerminal{X2}$ & 
%     \emph{binary operation} \\
%     %hline
%     % &&\hl{should I add ternary operation to eqn?}&&\\
    
%     $\nonTerminal{op}$ & $\vcentcolon=$ &
%     $op_= | op_\neq | op_> | op_\geq | op_< | op_\leq$ & 
%     \checkStyle{==} | \checkStyle{!=} | \checkStyle{>} | \checkStyle{>=} | \checkStyle{<} | \checkStyle{<=} & 
%     \emph{binary operator} \\
    
%     \hline
%     \multicolumn{5}{|c|}{Numeric Part}\\
%     \hline
    
%     $\nonTerminal{X_n} $ & $\vcentcolon=$ & 
%     $\nonTerminal{t}$ & 
%     $\nonTerminal{t}$ & 
%     \emph{numeric term}\\
%     & $|$ & 
%     $\nonTerminal{f_{op}} (\nonTerminal{X_1}, \nonTerminal{X_2})$ &
%     $\nonTerminal{X_1}\nonTerminal{f_{op}}\nonTerminal{X_2}$ & 
%     \emph{arithmetic operation} \\
    
%     %hline
    
%     $\nonTerminal{f_{op}}$ & $\vcentcolon=$ &
%     $f_{add} | f_{sub} | f_{mul} | f_{div}$ &
%     \checkStyle{+} | \checkStyle{-} | \checkStyle{*} | \checkStyle{/} &
%     \emph{arithmetic operator} \\
%     %hline
%     % & $|$ & $t_1$ mod $t_2$ & \checkStyle{t1\%t2} & \emph{modulo} \\
%     % & $|$ & $X_{m1} \stackrel{X}{=} X_{m2}$ & \checkStyle{Xm1==Xm2} & \emph{equality} \\
%     % & $|$ & $X_{m1} \stackrel{X}{\neq} X_{m2}$ & \checkStyle{Xm1!=Xm2} & \emph{inequality} \\
    
%     $\nonTerminal{t} $ & $\vcentcolon=$ & 
%     $x | x \in \mathbb{R} $ & 
%     $x$ & 
%     \emph{numeric literal}\\
    
%     & $|$ & 
%     $v : \termClass{TN}{v}$ & 
%     $v$ & 
%     \emph{numeric variable} \\
%     % & $|$ & $v_{unfilled}$ & \checkStyle{vunfilled} & \emph{(numeric) undefined variable} \\
%     \end{tabular}
%     % \todo[inline,color=yellow]{Interesting and important difference: You dont want "filled" and "unfilled" to be the part of the syntax, you just want to use them during evaluation }
%     \caption{Syntax of the input language}
%     \label{tab:syntax}
% \end{table*}
  
% \begin{table*}[h]
%     \centering
%     \begin{tabular}{r@{ }r@{ }c|c|l}
    
%     & & Check Syntax & Math. Syntax  & \\
    
%     \hline
%     \multicolumn{5}{|c|}{Pattern Structure Part}\\
%     \hline
    
%     % && \hl{We can probably rename the "body" predicate}&\hl{Distinguish terminal from non-terminal symbols beter}&\\
%     % \hl{ex in Type check, C is not an arbitrary string, rather a specific class name}&\\
    
%     $\nonTerminal{\varphi}$ & $\vcentcolon=$ &
%     $\nonTerminal{annotation} \checkStyle{pattern} \nonTerminal{name} $ & 
%     $\dslStyle{P}(\nonTerminal{params}) \Leftrightarrow{} \nonTerminal{bodies}$&
%     \emph{pattern defn} \\
%     &&$\checkStyle{(} \nonTerminal{params} \checkStyle{)} \nonTerminal{bodies}$&&\\
    
%     %hline
    
%     $\nonTerminal{params}$ & $\vcentcolon=$ &
%     $\nonTerminal{param}$ & 
%     $\nonTerminal{param}$ & 
%     \emph{parameter} \\
%     & $|$ & 
%     $\nonTerminal{params}\checkStyle{, } \nonTerminal{param}$ &
%     $\nonTerminal{params}, \nonTerminal{param}$
%     & \emph{parameter set} \\
    
%     %hline
    
%     $\nonTerminal{param}$ & $\vcentcolon=$ &
%     $v$ & 
%     $v$ & 
%     \emph{variable} \\
%     & $|$ & 
%     $v \checkStyle{ : } \nonTerminal{\symbolClass{EClassifier}{}}$&
%     $\termClass{T}{v}$ \hl{add this in semantics for structural part?}& 
%      \emph{typed variable} \\
    
%     %hline
    
%     $\nonTerminal{bodies}$ & $\vcentcolon=$ &
%     $\checkStyle{\{} \nonTerminal{body} \checkStyle{\}}$ &
%     $\exists \nonTerminal{params} : \nonTerminal{body}$ & 
%      \emph{constraint} \\
%     & $|$ & 
%     $\checkStyle{\{} \nonTerminal{body} \checkStyle{\} or } \nonTerminal{bodies} $ &
%     $\exists \nonTerminal{params} : \nonTerminal{body} \:\vee \nonTerminal{bodies}$ & 
%     \emph{constraint sequence} \\
    
%     %hline
    
%     $\nonTerminal{body}$ & $\vcentcolon=$ &
%     $ \nonTerminal{constr} \checkStyle{;}$ &
%     $\nonTerminal{constr}$ & 
%     \emph{constraint body} \\
%     & $|$ & 
%     $\nonTerminal{constr} \checkStyle{;} \: \nonTerminal{body}$ &
%     $ \nonTerminal{constr} \wedge \nonTerminal{body}$ & 
%     \emph{disj. of constrain bodies} \\
    
%     %hline
    
%     $\nonTerminal{constr}$ & $\vcentcolon=$ & 
%     $\nonTerminal{StrConstr} | \nonTerminal{NumConstr}$ & 
%     $\nonTerminal{StrConstr} | \nonTerminal{NumConstr}$ & 
%     \emph{constraint types} \\
    
%     %hline
    
%     $\nonTerminal{StrConstr}$ & $\vcentcolon=$ &
%     $\nonTerminal{\symbolClass{T}{}} \checkStyle{(} \nonTerminal{p}\checkStyle{)}$ & 
%   $\termClass{T}{\nonTerminal{p}}$ & 
%     \emph{type check} \\
%     % & $|$ & $\termClass{N}{p}$ & \checkStyle{java N(p)} & \emph{primitive type check} \\
%     & $|$ & 
%     $\nonTerminal{\symbolClass{TC}{}} \checkStyle{.} \nonTerminal{\symbolClass{R}{}}    \checkStyle{(}\nonTerminal{p_1}\checkStyle{, }\nonTerminal{p_2}\checkStyle{)}$ &
%     $\termReference{R}{\nonTerminal{p_1}}{\nonTerminal{p_2}}$ &
%     \emph{reference and attribute check}\\
    
%     &&&\hl{ref/attr navig missing}&\\
% %    & $|$ & $\termClass{C}{p_1} \wedge \termReferenceInd{R}{p_1}{p_2}{1} \wedge \termReferenceInd{R}{p_2}{p_3}{2} \wedge \ldots \wedge \termReferenceInd{R}{p_n}{p_{n+1}}{n}$ & $\checkStyle{C.R1.R2. ... .Rn(}$\nonTerminal{p_1}$\checkStyle{, p(n+1))}$ & \emph{reference and attribute navigation}\\
%     & $|$ & 
%     $\nonTerminal{\symbolClass{TC}{}} \checkStyle{.} \nonTerminal{\symbolClass{R}{}}   \checkStyle{+(}\nonTerminal{p_1}\checkStyle{, }\nonTerminal{p_2}\checkStyle{)}$ &
%     $\termTCReference{R}{\nonTerminal{p_1}}{\nonTerminal{p_2}}$ &
%     \emph{ref and attr transitive closure}\\
    
%     & $|$ & 
%     \checkStyle{}$\nonTerminal{p_1}$\checkStyle{ == }$\nonTerminal{p_2}$\checkStyle{} | \checkStyle{}$\nonTerminal{p_1}$\checkStyle{ != }$\nonTerminal{p_2}$\checkStyle{} & 
%     $\nonTerminal{p_1} \dslEqualSymbol \nonTerminal{p_2} \: | \: \neg (\nonTerminal{p_1} \dslEqualSymbol \nonTerminal{p_2})$&
%     \emph{equivalence/inequivalence}\\
%     % & $|$ & $\neg (p_1 \dslEqualSymbol p_2)$ & \checkStyle{}$\nonTerminal{p_1}$\checkStyle{ != }$\nonTerminal{p_1}$\checkStyle{} & \emph{inequivalence}\\

%     & $|$ & 
%     $\checkStyle{find} \nonTerminal{Q} \checkStyle{(} \nonTerminal{binding} \checkStyle{)}$ \hl{unsure} & 
%     $Q(\nonTerminal{binding})$ & 
%     \emph{pattern match}\\
%     & $|$ & 
%     $\checkStyle{neg find} \nonTerminal{Q} \checkStyle{(} \nonTerminal{binding} \checkStyle{)}$ & 
%     $\forall \: \nonTerminal{binding} :\neg Q(\nonTerminal{binding})$ & 
%     \emph{negated pattern match} \\
%     & $|$ & 
%     $\checkStyle{find} \nonTerminal{Q} \checkStyle{+(} \nonTerminal{bind_v} \checkStyle{)}$ & 
%     $Q^+(\nonTerminal{p_1}, \nonTerminal{p_2})$ & 
%     \emph{pattern transitive closure}\\

%     & $|$ & 
%     $\nonTerminal{constr_1}\checkStyle{?} \nonTerminal{constr_2} \checkStyle{:} \nonTerminal{constr_3}$ & 
%     $(\nonTerminal{constr_1} \wedge \nonTerminal{constr_2}) \vee $ & 
%     \emph{ternary operation} \\
%     && $(\neg \nonTerminal{constr_1} \wedge \nonTerminal{constr_3})$&&\\
    
%     %hline
    
%     % & $|$ & $body_1 \wedge body_2$ &  $\nonTerminal{body1}$ \checkStyle{;} $\nonTerminal{body2}$ \checkStyle{;} & \emph{constraint conjunction} \\
%     $\nonTerminal{binding}$ & $\vcentcolon=$ &
%     $\nonTerminal{p}$ & 
%     $\nonTerminal{p}$ & 
%     \emph{parameter} \\
%     & $|$ & 
%     $\nonTerminal{p}\checkStyle{, } \nonTerminal{binding}$ &
%     $\nonTerminal{p}, \nonTerminal{binding}$ & 
%      \emph{parameter set} \\
    
%     %hline
    
%     $\nonTerminal{p_n}$ & $\vcentcolon=$ & 
%     $\nonTerminal{\symbolClass{c}{}}$ & 
%     $c$ & 
%     \emph{metamodel literal}\\
%     & $|$ & 
%     $v$ & 
%     $v$ & 
%     \emph{variable}\\
    
%     %hline
    
%     $\nonTerminal{annotation}$ & $\vcentcolon=$ &
%     $\checkStyle{@Constraint} | \checkStyle{@QueryBasedFeature} | \epsilon$ &
%     & \emph{annotation defn} \\
%     %hline
%     $\nonTerminal{name}$ & $\vcentcolon=$ &
%     $\emph{EString}$ &
%     & \emph{name defn} \\
    
%     \hline
%     \multicolumn{5}{|c|}{Logical Evaluation of Check Expression}\\
%     \hline
    
%     $\nonTerminal{NumConstr}$ & $\vcentcolon=$ &
%     $\termClass{H}{binding} \Leftrightarrow{} \nonTerminal{eqn} $ & 
%     $\checkStyle{check(} \nonTerminal{eqn} \checkStyle{)}$ & 
%     \emph{predicate evaluation} \\
%     %hline
%     $\nonTerminal{eqn}$ & $\vcentcolon=$ &
%     % $\nonTerminal{op}(\nonTerminal{X_1}, \nonTerminal{X_2})$ & 
%     $\nonTerminal{X_1} \nonTerminal{op} \nonTerminal{X_2}$ & 
%     $\nonTerminal{X1} \nonTerminal{op} \nonTerminal{X2}$ & 
%     \emph{binary operation} \\
%     %hline
%     % &&\hl{should I add ternary operation to eqn?}&&\\

%     $\nonTerminal{op}$ & $\vcentcolon=$ &
%     % $op_= | op_\neq | op_> | op_\geq | op_< | op_\leq$ & 
%     $== | != | > | >= | < | <=$ & 
%     \checkStyle{==} | \checkStyle{!=} | \checkStyle{>} | \checkStyle{>=} | \checkStyle{<} | \checkStyle{<=} & 
%     \emph{binary operator} \\
    
%     \hline
%     \multicolumn{5}{|c|}{Numeric Part}\\
%     \hline
    
%     $\nonTerminal{X_n} $ & $\vcentcolon=$ & 
%     $\nonTerminal{t}$ & 
%     $\nonTerminal{t}$ & 
%     \emph{numeric term}\\
%     & $|$ & 
%     % $\nonTerminal{f_{op}} (\nonTerminal{X_1}, \nonTerminal{X_2})$ &
%     $ \nonTerminal{X_1} \nonTerminal{f_{op}} \nonTerminal{X_2}$ &
%     $\nonTerminal{X_1}\nonTerminal{f_{op}}\nonTerminal{X_2}$ & 
%     \emph{arithmetic operation} \\
    
%     %hline
    
%     $\nonTerminal{f_{op}}$ & $\vcentcolon=$ &
%     % $f_{add} | f_{sub} | f_{mul} | f_{div}$ &
%     $+ | - | \times | \div$&
%     \checkStyle{+} | \checkStyle{-} | \checkStyle{*} | \checkStyle{/} &
%     \emph{arithmetic operator} \\
%     %hline
%     % & $|$ & $t_1$ mod $t_2$ & \checkStyle{t1\%t2} & \emph{modulo} \\
%     % & $|$ & $X_{m1} \stackrel{X}{=} X_{m2}$ & \checkStyle{Xm1==Xm2} & \emph{equality} \\
%     % & $|$ & $X_{m1} \stackrel{X}{\neq} X_{m2}$ & \checkStyle{Xm1!=Xm2} & \emph{inequality} \\
    
%     $\nonTerminal{t} $ & $\vcentcolon=$ & 
%     $x | x \in \mathbb{R} $ & 
%     $x$ & 
%     \emph{numeric literal}\\
    
%     & $|$ & 
%     $v : \termClass{TN}{v}$ & 
%     $v$ & 
%     \emph{numeric variable} \\
%     % & $|$ & $v_{unfilled}$ & \checkStyle{vunfilled} & \emph{(numeric) undefined variable} \\
%     \end{tabular}
%     % \todo[inline,color=yellow]{Interesting and important difference: You dont want "filled" and "unfilled" to be the part of the syntax, you just want to use them during evaluation }
%     \caption{Syntax of the input language}
%     \label{tab:syntax}
% \end{table*}




\begin{table*}[h]
    \centering
    \begin{tabular}{r@{ }r@{ }c|c|l}
    
    & & Check Syntax & Math. Syntax  & \\
    
    \hline
    \multicolumn{5}{|c|}{Pattern Structure Part}\\
    \hline
    
    $\nonTerminal{\varphi}$ & $\vcentcolon=$ &
    $\nonTerminal{annotation} \checkStyle{pattern} \nonTerminal{name} $ & 
    $\termClass{P}{\nonTerminal{params}} \Leftrightarrow{} \nonTerminal{bodies}$&
    \emph{Structural predicate defn} \\
    &&$\checkStyle{(} \nonTerminal{params} \checkStyle{)} \nonTerminal{bodies}$&&\\
    
    $\nonTerminal{params}$ & $\vcentcolon=$ &
    $v$ & 
    $v$ & 
    \emph{variable} \\
    
    & $|$ & 
    $\nonTerminal{params}\checkStyle{, } v$ &
    $\nonTerminal{params}, v$
    & \emph{parameter set} \\
    
    &&&\hl{got rid of typed var in params}&\\
    
    % $\nonTerminal{param}$ & $\vcentcolon=$ &
    % $v$ & 
    % $v$ & 
    % \emph{variable} \\
    % & $|$ & 
    % $v \checkStyle{ : } \nonTerminal{\symbolClass{EClassifier}{}}$&
    % $\termClass{T}{v}$ \hl{add this in semantics for structural part?}& 
    %  \emph{typed variable} \\
    
    $\nonTerminal{bodies}$ & $\vcentcolon=$ &
    $\checkStyle{\{} \nonTerminal{body} \checkStyle{\}}$ &
    $\exists \nonTerminal{params} : \nonTerminal{body}$ & 
     \emph{constraint} \\
    & $|$ & 
    $\checkStyle{\{} \nonTerminal{body} \checkStyle{\} or } \nonTerminal{bodies} $ &
    $\exists \nonTerminal{params} : \nonTerminal{body} \:\vee \nonTerminal{bodies}$ & 
    \emph{constraint sequence} \\
    
    $\nonTerminal{body}$ & $\vcentcolon=$ &
    $ \nonTerminal{constr} \checkStyle{;}$ &
    $\nonTerminal{constr}$ & 
    \emph{constraint body} \\
    & $|$ & 
    $\nonTerminal{constr} \checkStyle{;} \: \nonTerminal{body}$ &
    $ \nonTerminal{constr} \wedge \nonTerminal{body}$ & 
    \emph{disj. of constrain bodies} \\
    
    $\nonTerminal{constr}$ & $\vcentcolon=$ & 
    $\nonTerminal{StrConstr} | \nonTerminal{NumConstr}$ & 
    $\nonTerminal{StrConstr} | \nonTerminal{NumConstr}$ & 
    \emph{constraint types} \\
    
    
    &&&\hl{got rid of constans c cuz not in 2.2.1}&\\
    
    $\nonTerminal{StrConstr}$ & $\vcentcolon=$ &
    $\nonTerminal{\symbolClass{T}{}} \checkStyle{(} v \checkStyle{)}$ & 
   $\termClass{T}{v}$ & 
    \emph{type check} \\
    & $|$ & 
    $\nonTerminal{\symbolClass{T}{}} \checkStyle{.} \nonTerminal{\symbolClass{R}{}}    \checkStyle{(}v_1\checkStyle{, }v_2\checkStyle{)}$ &
    $\termReference{R}{v_1}{v_2}$ &
    \emph{reference and attribute check}\\
    
    &&&\hl{ref/attr navig missing}&\\
    & $|$ & 
    $\nonTerminal{\symbolClass{T}{}} \checkStyle{.} \nonTerminal{\symbolClass{R}{}}   \checkStyle{+(}v_1\checkStyle{, }v_2\checkStyle{)}$ &
    $\termTCReference{R}{v_1}{v_2}$ &
    \emph{ref and attr transitive closure}\\
    
    & $|$ & 
    \checkStyle{}$v_1$\checkStyle{ == }$v_2$\checkStyle{} | \checkStyle{}$v_1$\checkStyle{ != }$v_2$\checkStyle{} & 
    $v_1 \dslEqualSymbol v_2 \: | \: \neg (v_1 \dslEqualSymbol v_2)$&
    \emph{equivalence/inequivalence}\\

    & $|$ & 
    $\checkStyle{find } \dslStyle{P} \checkStyle{(} \nonTerminal{params} \checkStyle{)}$ & 
    $\termClass{P}{\nonTerminal{params}}$ & 
    \emph{pattern match}\\
    & $|$ & 
    $\checkStyle{neg find } \dslStyle{P} \checkStyle{(} \nonTerminal{params} \checkStyle{)}$ & 
    $\forall \: \nonTerminal{params} :\neg \termClass{P}{\nonTerminal{params}}$ & 
    \emph{negated pattern match} \\
    & $|$ & 
    $\checkStyle{find } \dslStyle{P} \checkStyle{+(} v_1, v_2 \checkStyle{)}$ & 
    $\dslStyle{P}^+(v_1, v_2)$ & 
    \emph{pattern transitive closure}\\

    % & $|$ & 
    % $\nonTerminal{constr_1}\checkStyle{?} \nonTerminal{constr_2} \checkStyle{:} \nonTerminal{constr_3}$ & 
    % $(\nonTerminal{constr_1} \wedge \nonTerminal{constr_2}) \vee $ & 
    % \emph{ternary operation} \\
    % &&& $(\neg \nonTerminal{constr_1} \wedge \nonTerminal{constr_3})$&\\
    &&&\hl{got rid of binding cuz =params now}&\\
    % $\nonTerminal{binding}$ & $\vcentcolon=$ &
    % $\nonTerminal{p}$ & 
    % $\nonTerminal{p}$ & 
    % \emph{parameter} \\
    % & $|$ & 
    % $\nonTerminal{p}\checkStyle{, } \nonTerminal{binding}$ &
    % $\nonTerminal{p}, \nonTerminal{binding}$ & 
    %  \emph{parameter set} \\
    
    
    % $\nonTerminal{p_n}$ & $\vcentcolon=$ & 
    % $\nonTerminal{\symbolClass{c}{}}$ & 
    % $c$ & 
    % \emph{metamodel literal}\\
    % & $|$ & 
    % $v$ & 
    % $v$ & 
    % \emph{variable}\\
    
    
    $\nonTerminal{annotation}$ & $\vcentcolon=$ &
    $\checkStyle{@Constraint} | \checkStyle{@QueryBasedFeature} | \epsilon$ &
    & \emph{annotation defn} \\
    $\nonTerminal{name}$ & $\vcentcolon=$ &
    $\emph{EString}$ &
    & \emph{name defn} \\
    
    \hline
    \multicolumn{5}{|c|}{Logical Evaluation of Check Expression}\\
    \hline
    
    $\nonTerminal{NumConstr}$ & $\vcentcolon=$ &
    $\checkStyle{check(} \nonTerminal{eqn} \checkStyle{)}$ & 
    $\termClass{A}{binding} \Leftrightarrow{} \nonTerminal{eqn} $ & 
    \emph{Num. Attr. pred. defn} \\
    
    $\nonTerminal{eqn}$ & $\vcentcolon=$ &
    $\nonTerminal{X_1} \nonTerminal{op} \nonTerminal{X_2}$ & 
    $\nonTerminal{X_1} \nonTerminal{op} \nonTerminal{X_2}$ & 
    \emph{binary operation} \\

    $\nonTerminal{op}$ & $\vcentcolon=$ &
    \checkStyle{==} | \checkStyle{!=} | \checkStyle{>} | \checkStyle{>=} | \checkStyle{<} | \checkStyle{<=} & 
    $= | \neq | > | \geq | < | \leq$ & 
    \emph{binary operator} \\
    
    \hline
    \multicolumn{5}{|c|}{Numeric Part}\\
    \hline
    
    $\nonTerminal{X} $ & $\vcentcolon=$ & 
    $\nonTerminal{e}$ & 
    $\nonTerminal{e}$ & 
    \emph{numeric expression}\\
    & $|$ & 
    $ \nonTerminal{X} \nonTerminal{f_{op}} \nonTerminal{e}$ &
    $\nonTerminal{X}\nonTerminal{f_{op}}\nonTerminal{e}$ & 
    \emph{arithmetic operation} \\
    
    %hline
    
    $\nonTerminal{f_{op}}$ & $\vcentcolon=$ &
    $+ | - | \times | \div$&
    \checkStyle{+} | \checkStyle{-} | \checkStyle{*} | \checkStyle{/} &
    \emph{arithmetic operator} \\
    
    $\nonTerminal{e} $ & $\vcentcolon=$ & 
    $c$ & 
    $c$ & 
    \emph{constant symbol (literal)}\\
    
    & $|$ & 
    $v$& 
    $v$ & 
    \emph{numeric variable} \\
    \end{tabular}
    \caption{Syntax of the input language}
    \label{tab:syntax}
\end{table*}

\begin{table}[h]
    \centering
    \begin{tabular}{r@{ }r@{ }l}
    
    \hline
    \multicolumn{3}{|c|}{Pattern Structure Part}\\
    \hline
    
     \multicolumn{3}{c}{As defined in ICSE2018}\\
    $\semantics{\termClass{T}{v}}{P}{Z}$ & $\vcentcolon=$ &
    $\interpretationApp{P}{\symbolClass{T}{}}{Z(v)}$\\
    $ \semantics{\termHyperedge{P}{v_1}{v_n}}{P}{Z}$ & $\vcentcolon=$ &
    $\interpretationApp{P}{\symbolRef{P}{}}{Z(v_1), \ldots,  Z(v_2)}$  \\ 
    $\semantics{a \Leftrightarrow{} b}{P}{Z}$ & $\vcentcolon=$ &
    $\semantics{a}{P}{Z} == \semantics{b}{P}{Z}$\\
    
    \hline
    \multicolumn{3}{|c|}{Logical Evaluation of Check Expression}\\
    \hline
    
    $ \semantics{\termHyperedge{A}{v_1}{v_n}}{P}{Z}$ & $\vcentcolon=$ &
    $\interpretationApp{P}{\symbolRef{A}{}}{Z(p_1), \ldots,  Z(p_2)}$  \\ 
    
    $\semantics{X_1 \nonTerminal{op} X_2 | \numsems{X_1}{P}{Z} = \unbound \vee \numsems{X_2}{P}{Z} = \unbound}{P}{Z}$ & $\vcentcolon=$ & $\unk$\\
    $\semantics{X_1 \nonTerminal{op} X_2 | \numsems{X_1}{P}{Z}\neq \unbound \wedge \numsems{X_2}{P}{Z} \neq \unbound}{P}{Z}$ & $\vcentcolon=$ & $\numsems{X_1}{P}{Z} \: \nonTerminal{op} \: \numsems{X_2}{P}{Z}$\\
    % $\semantics{X_1 \neq X_2}{P}{Z}$ & $\vcentcolon=$ & $\numsems{X_1}{P}{Z}\neq \numsems{X_2}{P}{Z}$\\
    % $\semantics{X_1 > X_2}{P}{Z}$ & $\vcentcolon=$ & $\numsems{X_1}{P}{Z} > \numsems{X_2}{P}{Z}$\\
    % $\semantics{X_1 \geq X_2}{P}{Z}$ & $\vcentcolon=$ & $\numsems{X_1}{P}{Z} \geq \numsems{X_2}{P}{Z}$\\
    % $\semantics{X_1 < X_2}{P}{Z}$ & $\vcentcolon=$ & $\numsems{X_1}{P}{Z} < \numsems{X_2}{P}{Z}$\\
    % $\semantics{X_1 \leq X_2}{P}{Z}$ & $\vcentcolon=$ & $\numsems{X_1}{P}{Z} \leq \numsems{X_2}{P}{Z}$\\
    \hline
    \multicolumn{3}{|c|}{Numeric Part}\\
    \hline
    % $\numsems{t}{P}{Z}$ & $\vcentcolon=$ & $\numsems{t}{P}{Z}$ \hl{circular}\\
    $\numsems{X_1 \nonTerminal{f_{op}} X_2 | \numsems{X_1}{P}{Z} =  \unbound \vee \numsems{X_2}{P}{Z} = \unbound}{P}{Z}$ & $\vcentcolon=$ & $\unbound$\\
    $\numsems{X_1 \nonTerminal{f_{op}} X_2 | \numsems{X_1}{P}{Z}\neq \unbound \wedge \numsems{X_2}{P}{Z} \neq \unbound}{P}{Z}$ & $\vcentcolon=$ & $\numsems{X_1}{P}{Z} \: \nonTerminal{f_{op}} \: \numsems{X_2}{P}{Z}$\\
    $\numsems{X_1 \times X_2 | \numsems{X_1}{P}{Z} =  0 \vee \numsems{X_2}{P}{Z} = 0}{P}{Z}$ & $\vcentcolon=$ & $0$ \hl{is this necessary?}\\
    % $\numsems{\div(t_1, t_2)}{P}{Z}$ & $\vcentcolon=$ & $0$\\
    % $\numsems{t_1 + t_2}{P}{Z}$ & $\vcentcolon=$ & $t_1+t_2$\\
    % $\numsems{t_1 - t_2}{P}{Z}$ & $\vcentcolon=$ & $t_1-t_2$\\
    % $\numsems{t_1 * t_2}{P}{Z}$ & $\vcentcolon=$ & $t_1*t_2$\\
    % $\numsems{t_1 / t_2}{P}{Z}$ & $\vcentcolon=$ & $t_1/t_2$\\
    
    % $\numsems{X}{P}{Z}$ & $\vcentcolon=$ & $\interpretationNumFun{P}{(Z(X))}$\\
    
    $\numsems{c | c \in \mathbb{R}}{P}{Z}$ & $\vcentcolon=$ & $c$ \\
    % $\numsems{v : \termClass{TN}{v} | \interpretationNumApp{P}{\symbolClass{TN}{}}{Z(v)} = \unbound}{P}{Z}$ & $\vcentcolon=$ & $v$ \\
    $\numsems{v}{P}{Z}$ & $\vcentcolon=$ & $\interpretationNumFun{P}(Z(v))$ \\
    
    % \todo[inline,color=yellow]{you dont need intervals in this paper, you are using numbers in a way that is different from Kristofs work. (it will have a unified theory, but it might be concise, so we can move that to the JOT paper). So for the sake of simplicity you can use filled / unfilled (?) }

    \end{tabular}
    \caption{Semantics of the language}
    \label{tab:semantic}
\end{table}

==> fnc/color-elim.tex <==

\definecolor{viatraEmphColor}{RGB}{0,80,125}
\definecolor{keywordcolor}{rgb}{0.5,0,0.1}
\definecolor{commentcolor}{rgb}{0,0.3,0.1}
\definecolor{stringcolor}{rgb}{0,0,1}


\definecolor{emphColor}{rgb}{0.1,0.1,0.1}  %grey

\definecolor{logsemColor}{RGB}{0,80,125}

\definecolor{numsemColor}{RGB}{204,100,0}

\definecolor{blue0}{HTML}{47BCFF}
\definecolor{blue1}{HTML}{009BF5}
\definecolor{blue2}{HTML}{0067A3}
\definecolor{blue3}{HTML}{003452}
\definecolor{car1}{RGB}{128,125,123}  %grey
\definecolor{car2}{RGB}{194,92,85}  %red
\definecolor{car3}{RGB}{75,119,157}  %blue



\definecolor{completed}{RGB}{51,153,102}
\newcommand*{\completed}[0]{{\color{completed}{Completed}}}

\definecolor{inProgress}{RGB}{196,196,35}
\newcommand*{\inProgress}[0]{{\color{inProgress}{In Progress}}}

\definecolor{notYetStarted}{RGB}{255,0,0}
\newcommand*{\notYetStarted}[0]{{\color{notYetStarted}{Not Yet Started}}}

==> fnc/notation-old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
% mathematical notations
%%%%%%%%%%%%%%%%%%%%%%%

% Viatra Syntax
\definecolor{keywordcolor}{rgb}{0.5,0,0.1}
\definecolor{commentcolor}{rgb}{0,0.3,0.1}
\definecolor{stringcolor}{rgb}{0,0,1}

% v1
%\definecolor{emphColor}{rgb}{0,0.1,0.49}
% \definecolor{logsemColor}{RGB}{141,160,203}
% \definecolor{numsemColor}{RGB}{102,194,165}
% v2
% \definecolor{emphColor}{RGB}{231,41,138}
% \definecolor{logsemColor}{RGB}{117,112,179}
% \definecolor{numsemColor}{RGB}{27,158,119}

% v3
% emphcolor = dslStyle
%\definecolor{emphColor}{RGB}{102,102,102}
% \definecolor{viatraEmphColor}{RGB}{8,118,181}

% \definecolor{viatraEmphColor}{rgb}{0,0.1,0.49}
\definecolor{viatraEmphColor}{RGB}{0,80,125}
\definecolor{emphColor}{rgb}{0.1,0.1,0.1}
\definecolor{logsemColor}{rgb}{0,0.1,0.49}
\definecolor{logsemColor}{RGB}{0,80,125}
\definecolor{numsemColor}{RGB}{204,100,0} %orange

%Proposed new
% \definecolor{emphColor}{RGB}{88,19,183} %purple
% \definecolor{logsemColor}{rgb}{0,0.1,0.49} %lighter blue
% \definecolor{z3semColor}{RGB}{204,100,0} %orange
% \definecolor{drealsemColor}{RGB}{164,2,5} %red

\let\subsectionautorefname\sectionautorefname

\lstdefinelanguage{viatra}
{morekeywords={@QueryBasedFeature,@Constraint,count,pattern,package,
    neg,find,import,true,false,or,check,job,action,state,severity,location,message,oclIsKindOf,self,exists,includes,invariant,class,private,epackage,java},
 emph={Pseudostate,Vertex,Region,Transition,Entry,Synchronization,State,RegularState,CompositeElement,Trigger,Guard,Action,Statechart,vertices,regions,source,target,incomingTransitions,trigger,guard,action,elements,newElements,PartialModel,open,must,may,var,element,transitions,FamilyTree,members,Member,parents,age,VisionBlocked,blockedBy,Actor,xPos,yPos,ySpeed,placedOn,Lane_Horizontal,length,width},
 emphstyle={\color{viatraEmphColor}},
 sensitive=true, morecomment=[l]{//}, morecomment=[s]{/*}{*/},
 morestring=[b]{"}
}
\lstdefinelanguage{macl}
{morekeywords={rule,to,query,bind,value,policy,by,default,resolution,user,group,allow,deny,select,where,is,bound,from,with,import,priority,obj,ref,attr,restrictive},
 sensitive=no,
 morecomment=[l]{//},
 morecomment=[s]{/*}{*/},
 morestring=[b]{"},
} 
\lstdefinestyle{viatrasmall}{
	basicstyle=\scriptsize\ttfamily,
	commentstyle=\color{commentcolor}\ttfamily,
	stringstyle=\color{stringcolor}\ttfamily,
	%frameround=tttt,
	captionpos=b,
	keywordstyle=\color{keywordcolor}\bfseries\ttfamily,
	showstringspaces=false,
	tabsize=2,
	language=viatra,
	escapeinside={(*@}{@*)}%,
	%breaklines=false
}
\lstdefinestyle{viatrabig}{
	basicstyle=\ttfamily,
	commentstyle=\color{commentcolor}\ttfamily,
	stringstyle=\color{stringcolor}\ttfamily,
	%frameround=tttt,
	captionpos=b,
	keywordstyle=\color{keywordcolor}\bfseries\ttfamily,
	showstringspaces=false,
	tabsize=2,
	language=viatra,
	escapeinside={(*@}{@*)}%,
	%breaklines=false
}
\newcommand{\viatraStyle}[1]{\lstinline[style=viatrabig]@#1@}
%dsl symbols

\newcommand{\logsemStyle}[1]{{\color{logsemColor}{#1}}}
\newcommand{\numsemStyle}[1]{{\color{numsemColor}{#1}}}

\newcommand{\tptpStyle}[1]{\texttt{#1}}
\newcommand{\figscale}[0]{.4}

\newcommand{\dslStyle}[1]{\texttt{\color{emphColor}{#1}}}
\newcommand{\dslStyleP}[1]{\texttt{#1}}
\newcommand{\dslObjectSet}[0]{\mathcal{O}}
\newcommand{\dslIdSet}[0]{\mathit{Id}}
\newcommand{\dslInstanceOf}[2]{\dslStyle{#1}(#2)}
\newcommand{\dslInReference}[3]{\dslStyle{#1}(#2,#3)}
\newcommand{\dslInPattern}[2]{\dslStyleP{#1}(#2)}
\newcommand{\patternDef}[0]{:=}
\newcommand{\dslVar}[1]{\mathit{#1}}
\newcommand{\dslTheory}[0]{\mathcal{T}}
\newcommand{\termDistinct}[1]{\mathit{dist}(#1)}

\newcommand{\todoSig}[1]{\todo[inline, color=red]{#1}}
\newcommand{\newContent}[1]{\todo[color=yellow]{New: #1}}

% \newcommand{\interpretation}[2]{{[\![ #1 ]\!]}^{#2}}
% \newcommand{\interpretationVariable}[3]{{[\![ #1 ]\!]}^{#2}_{#3}}
\newcommand{\dslObjectSetI}[1]{\dslObjectSet_{#1}}
\newcommand{\dslInterpretationDefinition}[1]{\mathcal{I}_{#1}}
\newcommand{\dslInstanceOfI}[3]{\interpretation{\dslInstanceOf{#1}{#2}}{#3}}
\newcommand{\dslInReferenceI}[4]{\interpretation{\dslStyle{#1}(#2,#3)}{#4}}

\newcommand{\symbolClass}[2]{\dslStyle{#1}_{#2}}
\newcommand{\symbolRef}[2]{\dslStyle{#1}_{#2}}
\newcommand{\symbolTCRef}[2]{\dslStyle{#1}_{#2}^+}
\newcommand{\symbolHyper}[2]{\dslStyle{#1}_{#2}}


%\newcommand{\solver}[1]{\textit{#1}}
\newcommand{\phaseName}{\underline{\textsc{Phase}}}
\newcommand{\phase}[1]{\underline{\textsc{Phase {#1}}}}
\newcommand{\experiment}[1]{\underline{\textsc{Exp {#1}}}}
\newcommand{\solver}[1]{{\small\textsf{#1}}}
\newcommand{\term}{}
\newcommand{\termClass}[2]{\termClassInd{#1}{#2}{}}
\newcommand{\termClassInd}[3]{\symbolClass{#1}{#3}(\termConstant{#2})}
\newcommand{\termLiteral}[2]{\termLiteralInd{#1}{#2}{}}
\newcommand{\termLiteralInd}[3]{{#1}_{#3}(\termConstant{#2})}
\newcommand{\termConstantInd}[2]{{#1}_{#2}}
\newcommand{\termConstant}[1]{{#1}}
\newcommand{\termTCReference}[3]{\termTCReferenceInd{#1}{#2}{#3}{}}
\newcommand{\termTCReferenceInd}[4]{\symbolTCRef{#1}{#4}(\termConstant{#2},\termConstant{#3})}
\newcommand{\termReference}[3]{\termReferenceInd{#1}{#2}{#3}{}}
\newcommand{\termReferenceInd}[4]{\symbolRef{#1}{#4}(\termConstant{#2},\termConstant{#3})}
\newcommand{\termHyperedge}[3]{\termHyperedgeInd{#1}{#2}{#3}{}}
\newcommand{\termHyperedgeInd}[4]{\symbolHyper{#1}{#4}(\termConstant{#2}, \ldots, \termConstant{#3})}

\newcommand{\termEquals}[2]{\dslEquals{#1}{#2}}
\newcommand{\termExist}[1]{\dslExist{#1}}
\newcommand{\fwd}[0]{\mathit{ref}}
\newcommand{\refinement}[2]{#1\sqsubseteq#2}

\newcommand{\nonTerminal}[1]{\langle {#1} \rangle}

\newcommand{\semantics}[3]{{{\color{logsemColor}{\llbracket}} #1 {\color{logsemColor}{\rrbracket}}}^{#2}_{#3}}
\newcommand{\numsems}[3]{{{\color{numsemColor}{\llparenthesis}} #1 {\color{numsemColor}{\rrparenthesis}}}^{#2}_{#3}}
\newcommand{\interpretationFun}[1]{\mathcal{I}_{#1}}
\newcommand{\interpretationNumFun}[1]{\mathcal{V}_{#1}}
\newcommand{\interpretationDef}[4]{\interpretationFun{#1}(#2): {#3} \rightarrow {#4}}
\newcommand{\interpretationNumDef}[4]{\interpretationNumFun{#1}(#2): {#3} \rightarrow {#4}}
\newcommand{\interpretationApp}[3]{\mathcal{I}_{#1}(#2)(#3)}
\newcommand{\interpretationNumApp}[3]{\mathcal{V}_{#1}(#2)(#3)}
\newcommand{\interpretationConst}[2]{\mathcal{I}_{#1}(#2)}
\newcommand{\interpretationNumConst}[2]{\mathcal{V}_{#1}(#2)}



% \newcommand{\logicModel}[2]{\langle {#1}, {#2} \rangle}
\newcommand{\logicModel}[3]{\langle {#1}, {#2}, {#3} \rangle}

\newcommand{\logicStyle}[1]{\texttt{\color{logsemColor}{#1}}}
\newcommand{\numStyle}[1]{\texttt{\color{numsemColor}{#1}}}

\newcommand{\true}[0]{\textup{\logicStyle{1}}}
\newcommand{\false}[0]{\textup{\logicStyle{0}}}
\newcommand{\unk}[0]{\logicStyle{\nicefrac{1}{2}}}
\newcommand{\unbound}{\textup{\numStyle{?}}}

\newcommand{\dslExistSymbol}[0]{{\color{emphColor}{\varepsilon}}}
\newcommand{\dslExist}[1]{\dslExistSymbol(#1)}
\newcommand{\dslEqualSymbol}[0]{{\color{emphColor}{\sim}}}
\newcommand{\dslEquals}[2]{#1\mathrel{\dslEqualSymbol}#2}

\newcommand{\allModels}[1]{\mathcal{M}_\mathit{#1}}

\newcommand{\arity}[1]{\alpha(#1)}
\DeclareMathSymbol{\qm}{\mathalpha}{operators}{"3F}
\DeclareMathAlphabet{\mathbbold}{U}{bbold}{m}{n}

\newcommand{\ite}[3]{#1\mathrel{\textsf{?}}#2 \mathrel{\textsf{\textbf{:}}} #3}

%%%%%%%%%%%%%%%%%%%%%%%
% Eval
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\fofaf}{FAF}
\newcommand{\objectPred}[1]{object(\termConstant{#1})}
\newcommand{\object}{object}
\newcommand{\rquestion}[1]{\textbf{\textsc{RQ}#1}}
\newcommand{\ranswer}[2]{%
\noindent
\begin{tabularx}{\linewidth}{|X|}\hline
\rquestion{#1}: \emph{
#2
}\\\hline
\end{tabularx}}

%%%%%%%%%%%%%%
% Attribute Handling Commands
%%%%%%%%%%%%%%

\newcommand{\fctName}[1]{\textbf{#1}}
\newcommand{\trueText}{\textit{true}}

\newcommand{\checkStyle}[1]{\textbf{\texttt{#1}}}
\newcommand{\emf}[1]{\textit{#1}}

\newcommand{\objVal}[1]{\textsf{#1}}
\newcommand{\objSMT}[1]{\textsc{#1}}
